Energy-Efficient Deflection-based On-chip Networks: Topology, Routing, Flow Control

As the number of cores scales to tens and hundreds, the energy consumption of routers across various types of on-chip networks in chip muiltiprocessors (CMPs) increases significantly. A major source of this energy consumption comes from the input buffers inside Network-on-Chip (NoC) routers, which are traditionally designed to maximize performance. To mitigate this high energy cost, many works propose bufferless router designs that utilize deflection routing to resolve port contention. While this approach is able to maintain high performance relative to its buffered counterparts at low network traffic, the bufferless router design suffers performance degradation under high network load. In order to maintain high performance and energy efficiency under both low and high network loads, this chapter discusses critical drawbacks of traditional bufferless designs and describes recent research works focusing on two major modifications to improve the overall performance of the traditional bufferless network-on-chip design. The first modification is a minimally-buffered design that introduces limited buffering inside critical parts of the on-chip network in order to reduce the number of deflections. The second modification is a hierarchical bufferless interconnect design that aims to further improve performance by limiting the number of hops each packet needs to travel while in the network. In both approaches, we discuss design tradeoffs and provide evaluation results based on common CMP configurations with various network topologies to show the effectiveness of each proposal.

==> old.tex <==

%%%%% OLD

Modern computing systems are overwhelmingly designed to move data to
computation. This design choice goes directly against at least three
key trends in computing that cause performance, scalability and energy
bottlenecks: (1)~data access is a key bottleneck
as many important applications are increasingly data-intensive, and memory bandwidth and energy do not scale well, (2)~energy consumption is a key limiter in almost all computing platforms, especially server and mobile systems, (3)~data movement, especially off-chip to on-chip, is very expensive in terms of bandwidth, energy and latency, much more so than
computation. These trends are especially severely-felt in the
data-intensive server and energy-constrained mobile systems of today.

At the same time, conventional memory technology is facing many
technology scaling challenges in terms of reliability, energy, and
performance. As a result, memory system architects are open to
organizing memory in different ways and making it more intelligent, at
the expense of higher cost. The emergence of 3D-stacked memory plus
logic, the adoption of error correcting codes inside the latest DRAM
chips, proliferation of different main memory standards and chips, specialized for different purposes (e.g., graphics, low-power, high bandwidth, low latency), and the necessity of designing new solutions to serious reliability and security issues, such as the RowHammer phenomenon,
are an evidence of this trend.
 
This chapter discusses recent research that aims to practically
enable computation close to data, an approach we call \emph{processing-in-memory} (PIM). PIM places computation
mechanisms in or near where the data is stored (i.e., inside the
memory chips, in the logic layer of 3D-stacked memory,
or in the memory controllers), so that data movement between the
computation units and memory is reduced or eliminated. While
the general idea of PIM is not new, we discuss motivating trends in
applications as well as memory circuits/technology that greatly exacerbate the need for enabling it in modern computing systems. We examine at least two promising new approaches to designing PIM systems to accelerate
important data-intensive applications: (1)~{\em processing using memory} by exploiting analog operational properties of DRAM chips to perform
massively-parallel operations in memory, with low-cost changes, (2)~{\em processing near memory} by exploiting 3D-stacked memory technology design to provide high memory bandwidth and low memory latency to in-memory logic. In both approaches, we describe and tackle relevant cross-layer research, design, and adoption
challenges in devices, architecture, systems, and programming
models. Our focus is {on} the development of in-memory processing
designs that can be adopted in real computing platforms at low cost. We conclude by discussing work on solving key challenges to the practical adoption of PIM.













Main memory, built using the Dynamic Random Access Memory
(DRAM) technology, is a major component in nearly all computing
systems, including servers, cloud platforms, mobile/embedded devices, and sensor systems. Across all of these systems,the data working set
sizes of modern applications are rapidly growing, while the need for fast analysis of such data is increasing. Thus, main memory is becoming an increasingly significant bottleneck across a wide variety of computing systems and applications~\cite{mutlu.imw13, mutlu.superfri15, dean2013tail, kanev.isca15, ferdman.asplos12, wang.hpca14, boroumand.asplos18, mutlu2019enabling, mutlu2019, mutlu2020vlsi, ghose2019processing, alser2020accelerating, cali2020genasm, koppula2019eden, kanellopoulos2019smash, oliveira2021pimbench}. 
%%%OM:
%\om{JUAN, please add our DAC 2019 short paper + our Micpro 2019 paper + our IEEE Micro ACcelerating Genome Analysis paper + IBM JRD 2019 + GenASM + EDEN + SMASH + our upcoming PIM WL paper to this reference block} %%% JGL: Done - PIM-benchmarks cited as SIGMETRICS 2021 paper.
Alleviating the main memory bottleneck requires the memory capacity,
energy, cost, and performance to all scale in an efficient manner across technology generations.
Unfortunately, it has become increasingly difficult in recent years, especially the past decade, to scale all of these dimensions~\cite{kang.memoryforum14, mutlu.imw13,
mutlu.superfri15, mckee.cf04,wilkes.can01,kim-isca2014,salp,yoongu-thesis,raidr,mutlu2017rowhammer,donghyuk-ddma,lee-isca2009,yoon2012row,yoon-taco2014,lim-isca09,
wulf1995hitting, chang.sigmetrics16, lee.hpca13, lee.hpca15,
chang.sigmetrics17, lee.sigmetrics17, luo2014characterizing,
luo.arxiv17,hassan2017softmc, chargecache, kevinchang-thesis, patel2017reaper, hasan2019crow, ghose2018vampire, kim2018solar, kim2020revisiting, mutlu2020retrospective, wang2018cal, mutlu2018recent, ghose2019demystifying}, and thus the main memory bottleneck has been worsening.
%%% OM:
%\om{JUAN: Please add Revisiting Rowhammer + REAPER + our RH TCAD 2019 paper, CROW ISCA 2019, Solar-DRAM ICCD 2018, CAL-DRAM MICRO 2018, + "Recent Advances in DRAM and Flash Memory Architectures" Invited Journal Issue, IPSI Transactions on Internet Research, July 2018 + VAMPIRE SIGMETRICS 2018 + Demystifying DRAM-Workload Interactions SIGMETRICS 2019 to this reference block }

A major reason for the main memory bottleneck is the high energy and latency cost
associated with \emph{data movement}.  In modern computers, to
perform any operation on data that resides in main memory, the processor must retrieve
the data from main memory. This requires the memory controller
to issue commands to a DRAM module across a relatively slow and power-hungry off-chip bus (known as the \emph{memory channel}).  The DRAM module sends the requested data across the memory
channel, after which the data is placed in the caches and registers.
The CPU can perform computation on the data once the data is
in its registers.  Data movement from
the DRAM to the CPU incurs long latency and consumes a significant
amount of energy~\cite{hashemi.isca16,cont-runahead, ahn.tesseract.isca15, ahn.pei.isca15,boroumand.asplos18, keckler2011gpus}. 
%%% OM:
%\om{JUAN: Also cite "GPUs and the future of parallel computing" here }
These costs are often exacerbated by the fact that much of the data brought
into the caches is \emph{not reused} by the
CPU~\cite{qureshi.isca07,qureshi-hpca07, ahn.tesseract.isca15, ahn.pei.isca15}, 
providing little benefit in
return for the high latency and energy cost. 
%\rachata{Should we also add that recent advances in memory technology (NVMs), while can potentially improve energy efficiency, does not bring down the cost of data transfer?}.

The cost of data movement is a fundamental issue with the
\emph{processor-centric} nature of contemporary computer systems.
The CPU is considered to be the master in the system, and
computation is performed only in the processor (and accelerators).  In contrast, data storage and communication units, including the main memory, are
treated as unintelligent workers that are incapable of computation. 
As a result of this processor-centric design paradigm, data moves
a lot in the system between the computation units and communication/
storage units so that computation can be done on it. With the increasingly \emph{data-centric}
nature of contemporary and emerging applications, the
processor-centric design paradigm leads to great
inefficiency in performance, energy and cost.
For
example, most of
the real estate within a single compute node is already dedicated to
handling data movement and storage (e.g., large caches, memory
controllers, interconnects, and main memory)~\cite{kumar.isscc2009,howard201048core,jowani2010x8664,gillespie2014steam,singh2017zen},  %\om{JUAN: Can we add more good citations?}
and our recent work shows that more than 62\% of the entire system energy of a mobile device is spent on data movement between the processor and the memory
hierarchy for widely-used mobile workloads~\cite{boroumand2016pim}.

The large overhead of data movement in modern systems along
with technology advances that enable better integration of memory
and logic have recently prompted the re-examination of an old idea
that we will generally call Processing in Memory (PIM). The key
idea is to place computation mechanisms in or near where the data
is stored (i.e., inside the memory chips, in the logic layer of 3D-stacked
memory, in the memory controllers, or inside large caches),
so that data movement between where the computation is done
and where the data is stored is reduced or eliminated, compared to
contemporary processor-centric systems. Processing-in-memory is also known as \emph{near-data processing} (NDP),
enables the ability to perform operations and execute software tasks either using (1)~the memory
itself, or (2)~some form of processing logic (e.g., accelerators,
simple cores, reconfigurable logic) inside the memory subsystem.

The idea of PIM has been around for at least five
decades\ch{~\cite{stone1970logic,shaw1981non,
    elliott1992computational, kogge1994execube, gokhale1995processing,
    patterson1997case, oskin1998active, kang2012flexram,
    Draper:2002:ADP:514191.514197, Mai:2000:SMM:339647.339673,
    elliott.dt99, riedel.1998, keeton.1998, kaxiras.1997,
    acharya.1998, jino1978magnetic, doty1980magnetic, bongiovanni1980magnetic}}. 
%%% OM:
%\om{JUAN: Can we add some more old papers, please.} %JGL: Three more old papers added.
However, past efforts were
{\em not} widely adopted for various reasons, including 1) the difficulty of
integrating processing elements with DRAM, 2) the lack of critical
memory-related scaling challenges that current technology and
applications face today, and 3) that the data movement bottleneck
was not as critical to system cost, energy and performance as it is
today. As a result of
advances in modern memory architectures, {e.g., the integration
  of logic and memory in a 3D-stacked manner}, various recent works
explore a range of PIM architectures for multiple different purposes
\rachata{(e.g., \cite{zhu2013accelerating, pugsley2014ndc, zhang.hpdc14,
  farmahini2015nda, ahn.tesseract.isca15, ahn.pei.isca15,
  loh2013processing, hsieh.isca16, pattnaik.pact16,
  DBLP:conf/isca/AkinFH15, impica, DBLP:conf/sigmod/BabarinsaI15,
  DBLP:conf/IEEEpact/LeeSK15, DBLP:conf/hpca/GaoK16, chi2016prime,
  gu.isca16, kim.isca16, asghari-moghaddam.micro16, boroumand2016pim,
  hashemi.isca16, cont-runahead, GS-DRAM, liu-spaa17, gao.pact15,
  guo2014wondp, sura.cf15, morad.taco15, hassan.memsys15, li.dac16,
  kang.icassp14, aga.hpca17, shafiee2016isaac, seshadri2013rowclone,
  Seshadri:2015:ANDOR, chang.hpca16, seshadri.arxiv16,
  seshadri.micro17, nai2017graphpim,kim.arxiv17,kim.bmc18, li.micro17,
  kim.sc17, boroumand.asplos18,cali2020genasm,fernandez2020natsa,singh2019napel,seshadri2020indram, wang2020figaro, gao2020computedram, rezaei2020nom}).} 
  %%% RA: Added 7 more references from 2020
  %%%ON: JUAN: Please add all works that come in 2019 and 2020 here. All our works on PIM and other works we like. for example: 1. In-DRAM bulk bitwise exe engine, 2. CoNDA, ISCA 2019, 3. MAPEL, 4. NERO, 5. NATSA, 6. GenASM, 7. GRIM-Filter, 8. FIGARO, 9. NoM, CAL 2020, 10. Our JRD and MICPRO papers, 11. D-Range, 12. DRAM Latency puf, 13. ComputeDRAM, 14. ... 
  We believe it is crucial to re-examine PIM today with a fresh perspective (i.e., with novel approaches and ideas), by exploiting new memory technologies, with realistic workloads and systems, and with a mindset to ease adoption and feasibility.

In this chapter, we explore two new approaches to enabling
processing-in-memory in modern systems. The first approach \emph{minimally changes memory chips} to perform simple yet powerful common operations that the chip is inherently efficient at or could be made efficient at performing~\cite{seshadri.bookchapter17, seshadri2013rowclone,chang.hpca16,kevinchang-thesis,seshadri.thesis16,Seshadri:2015:ANDOR, seshadri.arxiv16, seshadri.micro17, li.micro17,GS-DRAM, ghose.bookchapter19, ghose.bookchapter19.arxiv,deng.dac2018, seshadri2020indram, wang2020figaro, gao2020computedram, rezaei2020nom, ghose2019processing,xin2020elp2im,aga.hpca17,eckert2018neural,fujiki2019duality,kang.icassp14,li.dac16,angizi2018pima,angizi2018cmp,angizi2019dna,levy.microelec14,kvatinsky.tcasii14,shafiee2016isaac,kvatinsky.iccd11,kvatinsky.tvlsi14,gaillardon2016plim,bhattacharjee2017revamp,hamdioui2015memristor,xie2015fast,hamdioui2017myth,yu2018memristive}. 
%%% OM:
%\om{JUAN: Please also cite our IBM JRD paper. I did not see it in references.} % JGL-2020-10-25
%\om{JUAN: Please add: 1. In-DRAM Bulk Bitwise Execution Engine, 2. FIGARO, 3. ComputeDRAM, 4. NoM CAL 2020, ... and more  }
%\jgl{Add more.} %JGL-2020-10-28
We call this approach {\em processing using memory}~\cite{ghose2019processing, seshadri.bookchapter17, seshadri.bookchapter17.arxiv, seshadri2020indram}.
%%% OM:  
%\om{JUAN: Please also cite our IBM JRD paper.} % JGL-2020-10-25
Some solutions that fall under
this approach take advantage of the existing DRAM design to cleverly
and efficiently perform \emph{bulk operations} (i.e., operations on an
entire row of DRAM cells), such as bulk copy, data initialization, and
bitwise operations, using the analog operational principles of DRAM~\cite{seshadri2013rowclone,Seshadri:2015:ANDOR,seshadri.thesis16, seshadri.arxiv16,seshadri.micro17, seshadri.bookchapter17, seshadri.bookchapter17.arxiv, seshadri2020indram}.
%%%OM: 
%\om{JUAN: please cite vivek's works including our latest stuff} 
Other solutions take advantage of the analog operational principles of emerging non-volatile memory technologies to perform similar bulk operations~\cite{li.dac16} or other specialized computations like convolutions and matrix multiplications~\cite{angizi2018pima,angizi2018cmp,angizi2019dna,levy.microelec14,kvatinsky.tcasii14,shafiee2016isaac,kvatinsky.iccd11,kvatinsky.tvlsi14,gaillardon2016plim,bhattacharjee2017revamp,hamdioui2015memristor,xie2015fast,hamdioui2017myth,yu2018memristive,ankit2019puma}.
%%%OM:
%\om{Please add citations we have in the IBM JRD paper for taking advantage of emerging technologies to perform processing using memory.}. %JGL-2020-10-25

The second approach enables PIM in
a more general-purpose manner by taking advantage of computation capability in conventional memory controllers~\cite{hashemi.isca16,cont-runahead}
%%%OM:
%\om{Please cite Milad's ISCA 2016 and MICRO 2016 papers here. There may be more...} %JGL-2020-10-25
or the logic layer(s) of the relatively new \emph{3D-stacked memory technologies}~\cite{loh2013processing, pugsley2014ndc, zhu2013accelerating, DBLP:conf/isca/AkinFH15,impica, ahn.tesseract.isca15, nai2017graphpim, DBLP:conf/sigmod/BabarinsaI15, gao.pact15, kim.bmc18, kim.arxiv17, gu.isca16, boroumand2016pim, boroumand.asplos18, chi2016prime,  kim.isca16, DBLP:conf/IEEEpact/LeeSK15, ahn.pei.isca15, zhang.hpdc14, hsieh.isca16, pattnaik.pact16, sura.cf15, hassan.memsys15,farmahini2015nda, DBLP:conf/hpca/GaoK16,  guo2014wondp,liu-spaa17,kim.sc17,cali2020genasm,fernandez2020natsa,singh2019napel,singh2020nero}. 
%%% OM:
%\om{JUAN: PLease cite more in the preceding reference box. many to cite here.}
%\jgl{Add more.}\om{Add our works like NERO, NAPEL, ... Let's be comprehensive.} %JGL-2020-1025
We call this general approach {\em processing near memory}~\cite{ghose2019processing}. 
%\om{JUAN: Please cite our IBM JRD paper.}  %JGL-2020-10-25
This approach is especially catalyzed by recent advancements in 3D-stacked memory technologies that include a logic processing layer underneath memory layers~\cite{ramulator,lee.taco16}.
In order to stack multiple layers of memory, 3D-stacked chips use vertical \emph{through-silicon vias} (TSVs) to connect the layers to each other, and to the I/O drivers of the chip~\cite{lee.taco16}. 
The TSVs provide much greater \emph{internal} bandwidth within the 3D stack layers than is available externally on the memory
channel.  Several such 3D-stacked memory architectures, such as the
Hybrid Memory Cube~\cite{hmc.spec.1.1, hmc.spec.2.0} and
High-Bandwidth Memory~\cite{jedec.hbm.spec,lee.taco16}, include a
\emph{logic layer}, where designers can add some processing
logic (e.g., accelerators, simple cores, reconfigurable logic) to take advantage of this high internal bandwidth. Future die-stacking technologies, like {\em monolithic 3D}~\cite{gopireddy2019m3d,mitra2018vlse,hwang2018cmos,mitra2015nano,rich2020nano,sabry2015abundant,sabry2019n3xt},
%\om{cite several N3XT papers}, %JGL-2020-10-25
can amplify the benefits of this approach by greatly improving internal bandwidth and the number of logic layers between memory layers. 

Regardless of the approach taken to PIM, there are key practical
adoption challenges that system architects and programmers must
address to enable the widespread adoption of PIM across the computing
landscape and in different domains of workloads. In addition to describing work along
the two key approaches, we also discuss these challenges in work
paper, along with existing work that addresses these challenges.

Before we describe in detail the two modern approaches to PIM in Section~\ref{sec:pim}, we first describe major trends affecting main memory (Section~\ref{sec:majortrends}), then demonstrate  many reasons why we need to have intelligent memory controllers to enhance memory scaling into the future (Section~\ref{sec:intmemcont}), followed by an analysis of the major shortcomings of the processor-centric computing paradigm which PIM intends to augment, disrupt, and perhaps in some cases displace (Section~\ref{sec:processorcentric}).





\section{Major Trends Affecting Main Memory}
\label{sec:majortrends}
%\addcontentsline{toc}{part}{Major Trends Affecting Main Memory}


Main memory is a major, critical component of all computing
systems, including cloud and server platforms, desktop computers,
mobile and embedded devices, and sensors. It constitutes one of the main pillars of any computing platform, together with 1) the processing
elements (or computational elements), which can include CPU cores, GPU cores, accelerators, or reconfigurable devices, and 2) the communication elements, which can include interconnects, network interfaces, and network processing units.

Due to its relatively low cost and low latency, Dynamic Random Access Memory (DRAM)~\cite{dennard1968field}
%\om{JUAN: Please cite Dennard's seminal patent from 1965.} %JGL-2020-10-26
is the predominant data storage technology that is used to build main memory. The growing data working set sizes of modern applications~\cite{mutlu.imw13, mutlu.superfri15,dean2013tail, kanev.isca15, ferdman.asplos12,wang.hpca14, boroumand.asplos18,pekhimenko2012lcp,pekhimenko2013lcp,churin1988camac,abali2001mxt,friedrich2014power8}
%\om{JUAN: Please cite some memory compression papers as well: 1. Linearly Compressed Pages, 2. IBM XT memory controller, 3. IBM POWER8, and more.} %JGL-2020-10-26
impose an ever-increasing demand for higher DRAM capacity and performance. Unfortunately, DRAM technology scaling is becoming increasingly challenging: it is increasingly difficult to enlarge DRAM chip capacity at low cost while also maintaining maintain DRAM performance, energy efficiency, and reliability~\cite{liu.isca13,mutlu.imw13,kim-isca2014,mutlu2017rowhammer,ghose2018vampire,mutlu.superfri15,kim2020revisiting,mutlu2020retrospective,frigo2020trr}
%\om{JUAN: Add: 1. Our RowHammer TCAD 19 paper, 2. Revisiting RowHammer 2020, 3. TRRespass 2020, 4. Our SUPERFRI paper, 5..} %JGL-2020-10-26
Thus, fulfilling the increasing memory needs of modern workloads is becoming
increasingly costly and difficult~\cite{dean2013tail,kanev.isca15,mckee.cf04,mutlu.superfri15,wilkes.can01,salp,kang.memoryforum14,yoongu-thesis,raidr,ahn.tesseract.isca15,ahn.pei.isca15,hsieh.isca16,donghyuk-ddma,lee-isca2009,yoon2012row,yoon-taco2014,lim-isca09,wulf1995hitting,chang.sigmetrics16,lee.hpca13,lee.hpca15,chang.sigmetrics17,lee.sigmetrics17,luo2014characterizing,luo.arxiv17,hassan2017softmc,chargecache,wang2018cal,das.dac18,kim2018solar, kevinchang-thesis, wang2020figaro, kim2020revisiting, luo2020clr, koppula2019eden, mutlu2020retrospective, hasan2019crow, patel2019understanding, patel2020bit, ghose2019demystifying, kim.hpca19}.
%\om{JUAN: Please cite more here - our recent papers on DRAM in 2019, 2020 and other good papers.} %JGL-2020-10-26

If CMOS technology scaling is coming to an end~\cite{denning.2016},
the projections are significantly worse for DRAM technology
scaling~\cite{itrs.2009}. DRAM technology scaling affects all
  major characteristics of DRAM, including capacity,
bandwidth, latency, reliability, energy, and cost.  
We next describe the key issues and trends in DRAM technology scaling 
and discuss how these trends motivate the need for {\em intelligent memory controllers}, i.e., controllers that have intelligence and computation capability to enable better scaling of main memory in terms of all metrics of interest. Such intelligent memory controllers can also more easily pave the way to and be used as a starting substrate for processing in memory.

The first key {concern is the difficulty} of scaling DRAM
capacity (i.e., density, or cost per bit), bandwidth and latency {\em
  at the same time}.  
While the processing core count doubles every
two years, the DRAM capacity doubles only every three
years, as shown by~\cite{lim-isca09}, and the latter is slowing down. 
This trend causes the \emph{memory capacity per
  core} to drop by approximately 30\% every two
years~\cite{lim-isca09}. The trend is even worse for \emph{memory
  bandwidth per core} -- in the approximately two decades between 1999 and 2017, {DRAM chip storage capacity (for the most commonly-used DDRx chip of the time)} has improved
approximately 128$\times$ while DRAM bandwidth has improved only approximately
20$\times$~\cite{kevinchang-thesis,chang.sigmetrics16,lee.hpca13}, as shown in Figure~\ref{fig:dram-lat-band-cap}. In
the same period of about two decades, DRAM latency (as measured by the row
cycling time) has remained almost constant (i.e., reduced by only
30\%, as shown in Figure~\ref{fig:dram-lat-band-cap}), making it a significant performance bottleneck for {many
  modern workloads, including} in-memory
databases~\cite{ailamaki1999dbmss,boncz.1999,clapp.2015,JAFAR,boroumand2016pim,GS-DRAM,seshadri.micro17,boroumand2019conda},
%\om{JUAN: cite 1. Vivek GS-DRAM, 2. Vivek Ambit, 3. Amirali CoNDA, 4. Amirali LazyPIM}, %JGL-2020-10-26
graph processing~\cite{ahn.tesseract.isca15,umuroglu.2015,xu.2014,ahn.pei.isca15,kanellopoulos2019smash},
%\om{JUAN: cite 1. PEI, 2. SMASH}, %JGL-2020-10-26
data analytics~\cite{awan.2015,awan.2016,clapp.2015,yasin.2014}, datacenter workloads~\cite{kanev.isca15}, neural networks~\cite{koppula2019eden, chi2016prime, desa2018high, han2016eie, long2018reram, schuiki2018scalable, boroumand.asplos18},
%\om{JUAN: Add EDEN and key citations from EDEN here showing the importance of memory in evaluating NNs}, %JGL-2020-1026
and consumer workloads~\cite{boroumand.asplos18}. 
As low-latency computing is becoming ever more important~\cite{mutlu.imw13, mutlu.superfri15, cali2020genasm, cali2018nano, alser2020accelerating, alser.bioinformatics17, alser2020sneakysnake, alser2019shouji,dean2013tail},
%\om{JUAN: cite 1. our SUPERFRI paper, 2. GenASM, 3. Damla's nanopore paper in BIB, 4. Accelerating Genome Analysis, 5. Gatekeeper, 6. Shouji, 7. Sneakysnake, 8. Tail at Scale paper from Google, 9. add more papers showing the importance of low latency computing}, %JGL-2020-10-26
e.g., due to the ever-increasing need to process large amounts of data at real time, and predictable performance continues to be a critical concern in the design of modern computing systems~\cite{moscibroda-usenix2007,mutlu-micro2007,mutlu-isca2008,mutlu.superfri15,lavanya-thesis,donghyuk-ddma,subramanian-hpca2013,usui-taco2016,subramanian-micro2015,kim2010thread,kim2014bounding,kim2016bounding},
%\om{JUAN: cite 1. TCM, Micro 2010, 2. Our RTAS 2014 paper by Hyoseung Kim et al., 3. Our RTS Journal paper from 2016, 4. more works}, %JGL-2020-10-26
it is increasingly critical to design low-latency main memory chips.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/dram-lat-band-cap.pdf}
\vspace{-5mm}
\caption{Scaling of DRAM capacity, bandwidth and latency between 1999 and 2017, normalized to the value in 2017. Data depicted for the most common type of DDRx chip of each year. Reproduced from~\cite{mutlu.iccdtalk19}. Originally presented in~\cite{chang.sigmetrics16,chang.sigmetrics16talk,chang.phdthesis2017}.
%\om{JUAN: Please cite Kevin's SIGMETRICS 2016 paper and talk https://people.inf.ethz.ch/omutlu/pub/understanding-latency-variation-in-DRAM-chips_kevinchang_sigmetrics16-talk.pdf + Kevin's disssertation and link to PDF and slides from our PhD theses page}
%JGL-2020-11-02
}
\label{fig:dram-lat-band-cap}
\end{figure}


The second key concern is that DRAM technology scaling to
  smaller nodes adversely affects DRAM reliability.  A DRAM cell
stores one bit of data in the form of charge in a capacitor, which is
accessed via an access transistor and peripheral circuitry. For a DRAM
cell to operate correctly, both the capacitor and the access
transistor (as well as the peripheral circuitry) need to operate
reliably. As the size of the DRAM cell reduces, both the capacitor and
the access transistor become less reliable, more leaky, and generally more vulnerable to electrical noise and disturbance.  As a result,
{reducing the size of the DRAM cell} increases the difficulty of
correctly storing and detecting the desired original value in the DRAM, as shown in various recent works that study DRAM reliability by analyzing data retention and other reliability issues of modern DRAM chips
cell~\cite{liu.isca13,mutlu.imw13,kim-isca2014,mutlu2017rowhammer,khan.sigmetrics14, khan.dsn16, khan.cal16, khan.micro17, qureshi.dsn15, patel2017reaper, hassan2017softmc, hasan2019crow, raidr, patel2020bit, patel2019understanding, kim2020revisiting, mutlu2020retrospective, frigo2020trr, cojocar2020susceptible}.
%\om{JUAN: We should cite a lot more here. Basically, all our works on DRAM retention failures and RowHammer. Here is a starter list: 1. Samira SIGMETRICS 2014, DSN 2016, CAL 2016, MICRO 2017, 2. AVATAR DSN 2015, 3. REAPER ISCA 2017, 4. SoftMC HPCA 2017, 5. CROW, ISCA 2019, 6. RAIDR ISCA 2012, 7. minesh DSN 2019, MICRO 2020, 8. RevisitingRowHammer ISCA 2020, 9. RH TCAD 2019, 10. TRRespass SP 2020, 11. Our "Are we vulnerable to RH?" work with Microsoft in SP 2020, ...}. %JGL-2020-10-26
Hence, memory technology scaling causes memory errors to appear more frequently. For example, a study of Facebook's entire production datacenter servers
showed that memory errors, and thus the server failure rate, are strongly positively  correlated with the density of the chips employed in the
servers~\cite{meza.dsn15}: the higher the density of the chip used in a server, the more likely the server is to experience a memory error and server failure. Thus, it is critical to make the main memory
system more reliable to build reliable computing systems on top of it.


The third key {issue} is that the reliability problems caused by
aggressive DRAM technology scaling can lead to new security
vulnerabilities. {The RowHammer phenomenon}~\cite{kim-isca2014,mutlu2017rowhammer,mutlu2020retrospective,kim2020revisiting}
  %\om{JUAN: Please add 1. Our TCAD 2019 paper, 2. revisiting Rowhammer ISCA 2020} %JGL-2020-10-26
shows that it is possible to {predictably} induce errors {(bit flips)} in most {modern} DRAM chips.  {Repeatedly reading the same row in DRAM can corrupt data in physically-adjacent rows. Specifically, when a DRAM row is opened (i.e., activated) and closed (i.e., precharged) repeatedly (i.e., hammered), enough times within a DRAM refresh interval, one or more bits in physically-adjacent DRAM rows can be flipped to the wrong value.  A very simple user-level program~\cite{rowhammer.github} can reliably and consistently induce RowHammer errors in vulnerable DRAM modules.}  {The seminal paper that introduced RowHammer~\cite{kim-isca2014} showed that more than 85\% of the chips tested, built by three major vendors between 2010 and 2014, were vulnerable to RowHammer-induced errors}. In particular, \emph{all} DRAM modules from 2012 and 2013 are vulnerable, as shown by the Figure~\ref{fig:rowhammer} which depicts the observed RowHammer error vulnerability of DRAM modules manufactured between 2008 and 2014 by all three major DRAM manufacturers A, B, C~\cite{kim-isca2014}. 
A recent technology scaling study~\cite{kim2020revisiting} 
%\om{JUAN: please cite revisiting Rowhammer ISCA 2020} %JGL-2020-10-26
of 1580 DRAM chips belonging to three different DRAM types and various different technology node sizes experimentally demonstrated that the RowHammer vulnerability is getting much worse at the circuit level: fewer number of activates to a row can cause bit flips in the most recent chips and recent chips experience higher bit flip rates due to RowHammer. The same work~\cite{kim2020revisiting} 
%\om{JUAN: please cite revisiting Rowhammer ISCA 2020} %JGL-2020-10-26
also showed that existing RowHammer mitigation mechanisms will not be effective in future DRAM chips that will be much more vulnerable to RowHammer, and thus RowHammer remains to be an open vulnerability to securely protect against.   

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/rowhammer.pdf}
\vspace{-5mm}
\caption{RowHammer vulnerability for DRAM modules manufactured between 2008 and 2014. Reproduced from~\cite{mutlu.nsfpim20}. Originally presented in~\cite{kim-isca2014,kim.isca2014talk}.
%\om{JUAN: Please cite our RH ISCA paper and Yoongu's ISCA 2014 talk}
%JGL-2020-11-02
}
\label{fig:rowhammer}
\end{figure}


The RowHammer {phenomenon} entails a real reliability, and
perhaps even more importantly, a real and prevalent security issue. It
breaks physical {memory} isolation between two addresses, one of
the fundamental building blocks of memory, on top of which system
security principles are built. With RowHammer, accesses to one row
(e.g., an application page) can modify data stored in another memory
row (e.g., an OS page).  This was confirmed in 2015 by researchers from Google Project Zero, who developed a user-level attack that uses RowHammer to
gain kernel privileges~\cite{seaborn.2015,seaborn.2016}.  Other
researchers have shown how RowHammer vulnerabilities can be exploited
in various ways to gain privileged access to various systems: in a
remote server RowHammer can be used to remotely take over the server
via the use of JavaScript~\cite{gruss.2015}; a virtual machine can
take over another virtual machine by inducing errors in the victim
virtual machine's memory space~\cite{razavi.2016}; a malicious
application without permissions can take control of an Android mobile
device~\cite{vanderveen.2016}; or an attacker can gain arbitrary
read/write access in a web browser on a Microsoft Windows 10
system~\cite{bosman.2016}. Over the past six years, many security attacks were developed to exploit RowHammer~\cite{cloudflops,bosman.2016,anotherflip,qiao2016new,bhattacharya2016curious,jang2017sgx,aga2017good,pessl2016drama,gruss.2015,razavi.2016,vanderveen.2016,glitch-vu,fournaris2017exploiting,poddebniak2018attacking,nethammer,throwhammer,tatar2018defeating,carre2018openssl,barenghi2018software,zhang2018triggering,bhattacharya2018advanced,cojocar19exploiting,seaborn.2015,seaborn.2016}.
%\om{JUAN: Please cite many security attack papers we cite in our TCAD 2019 paper with Jeremie. You can get the repo and the bib file from Jeremie and include the relevant references from there.}. %JGL-2020-10-27
Very recently, the TRRespass attack~\cite{frigo2020trr} %\om{JUAN: Please cite TRRespass} %JGL-2020-1026
showed that existing DRAM chips that are advertised to be RowHammer-resistant, as described by various DRAM vendors~\cite{lee2014green,micron2016ddr4},
%\om{JUAN: Please cite the references from the TRRespass paper that point to vendor statements} %JGL-2020-10-27
are actually vulnerable because these mitigation mechanisms can be circumvented with a new type of RowHammer attack called {\em many-sided hammering}. For a more detailed treatment of the
RowHammer problem and its consequences, as well as its root causes, modeling, and analyses, we refer the reader
to~\cite{kim-isca2014,mutlu2017rowhammer,rowhammer-topinhes18,mutlu2020retrospective,kim2020revisiting,frigo2020trr,cojocar2020susceptible}. %\om{JUAN: Add 1. TCAD 2019, 2. Revisiting RowHammer, 3. TRRespass, 4. Our SP paper with Microsoft}. %JGL-2020-10-26

The fourth key {issue} is the power and energy consumption of
main memory. DRAM is inherently a power and energy hog, as it consumes
energy even when it is not used (e.g., it requires periodic memory
refresh~\cite{raidr}), due to its charge-based nature. And, energy
consumption of main memory is becoming worse due to three major
reasons. First, main memory's capacity, bandwidth, parallelism, and complexity are all
increasing, causing energy consumption to naturally increase due to higher amount of dynamic activity and higher overall static power consumption. Second, main memory has remained off the main processing
chip and thus did not benefit from many energy reduction mechanisms that come with better integration, even though many other platform components have been integrated into the processing chip and have benefited from the aggressive energy/voltage  scaling mechanisms and the low-energy communication substrate on-chip. Third, the difficulties in DRAM technology scaling are making DRAM energy reduction very difficult with technology generations. In fact, some of the mechanisms that are added to DRAM chips to compensate for reliability problems in smaller technology generations, e.g., in-DRAM error correcting codes~\cite{patel2017reaper,patel2019understanding,patel2020bit,kang.memoryforum14,oh2014ecc,micron2017ecc,jedec2020ddr5}
%\om{JUAN: Please cite 1. Minesh's ISCA 2017, DSN 2019 and MICRO 2020 papers, 2. Uksong Kang's memory forum 2014 paper, 3. Papers from Samsung, Hynix and Micron saying they have in-DRAM ECC -- please ask Minesh or find them in his recent papers} 
and higher refresh rates~\cite{patel2020bit,kwak2017refresh,kwon2017wearable,apple2015about}, 
%\om{JUAN: cite LPDDR4 papers and Minesh's MICRO 2020 paper + ask Minesh}, 
directly increase energy consumption. As a result of these three major issues that make main memory a larger energy bottleneck, the fraction of the entire system power consumed by main memory is increasing over the last two decades. In 2003,
{Lefurgy et al.~\cite{lefurgy.2003} showed that, in
  large commercial servers designed by IBM, the off-chip memory
  hierarchy (including, at that time, DRAM, interconnects, memory
  controller, and off-chip caches) consumed between 40\% and 50\% of
  the total system energy. The trend has become even worse over the
  course of the one-to-two decades.}  In recent computing systems with
CPUs or GPUs, {\em only DRAM itself} is shown to account for more
than 40\% of the total system power~\cite{ware.2010,paul.2015,chang.sigmetrics17,ghose2018vampire}.
%\om{JUAN: cite 1. Kevin Chang SIGMETRICS 2017, 2. Saugata VAMPIRE SIGMETRICS 2018} %JGL-2020-10-27
Hence, the power and energy consumption of main memory is increasing relative
to that of other components in computing platform. As energy
efficiency and sustainability are critical necessities in computing
platforms today, it is critical to reduce the energy and power
consumption of main memory~\cite{david2011memdvfs,deng2011memscale,chang.sigmetrics17,ghose2018vampire,haj2020sysscale,haj2020techniques,ghose2019demystifying}.
%\om{JUAN: cite 0. David+ MemDVFS ICAC 2011, 1. Kevin Chang SIGMETRICS 2017, 2. Saugata VAMPIRE SIGMETRICS 2018, 3. Saugata Demystifying ... SIGMETRICS 2019, 4. Jawad HPCA 2020 and ISCA 2020 papers, 5. MemScale ASPLOS 2011} . %JJGL-2020-10-27



\section{The Need for Intelligent Memory Controllers to Enhance Memory Scaling}
\label{sec:intmemcont}
%\addcontentsline{toc}{part}{The Need for Intelligent Memory Controllers to Enhance Memory Scaling}

A key promising approach to solving the four major issues above is to
design {\em intelligent memory controllers} that can manage main
memory better. If the memory controller is designed to be more
intelligent and more programmable, it can, for example, incorporate
flexible mechanisms to overcome various types of reliability issues
(including RowHammer), manage latencies and energy/power consumption better
based on a deep understanding of the DRAM chip and application
characteristics, provide enough support for programmability to prevent
security and reliability vulnerabilities that are discovered in the
field, and manage various types of memory technologies that are put
together as a hybrid main memory to enhance the scaling of the main
memory system. We provide a few examples of how an intelligent memory
controller can help overcome circuit- and device-level issues modern computing systems are
facing at the main memory level. We believe having intelligent memory
controllers can greatly alleviate the scaling issues encountered with
main memory today, as we have described in an earlier position
paper~\cite{mutlu.imw13}. This is a direction that is also supported
by key hardware manufacturers in computing industry today, as described in an informative paper written
collaboratively by Intel and Samsung engineers on DRAM technology
scaling issues\sg{~\cite{kang.memoryforum14}}.

In this section, we give several examples of how an intelligent memory controller can help overcome major scaling challenges of modern DRAM.   
First, a slightly more intelligent memory controller than today's controllers can prevent the RowHammer vulnerability by
probabilistically refreshing rows that are physically adjacent to an activated row, with a very low probability. This solution, called PARA
(Probabilistic Adjacent Row Activation)~\cite{kim-isca2014} was shown
to provide strong, programmable, robust guarantees against RowHammer, with
very little power, performance and chip area
overheads~\cite{kim-isca2014}. It requires a slightly more intelligent
memory controller that 1) knows (or that can figure out) the physical
adjacency of rows in a DRAM chip, 2) is programmable enough to
adjust the probability of adjacent row activation depending on the vulnerability of a chip, and 3) can issue refresh
requests to physically-adjacent rows accordingly to the probability supplied by
the system or discovered online. As described by prior
work~\cite{kim-isca2014,mutlu2017rowhammer,rowhammer-topinhes18,mutlu2020retrospective,kim2020revisiting},
%\om{JUAN: please cite TCAD 2019 and Revisiting RowHammer}, %JGL-2020-1026
this solution has much lower performance and energy overheads than \sg{increasing the} refresh rate across
the board for the entire main memory, which is the RowHammer solution
employed by existing systems in the field that have simple and rigid
memory controllers~\cite{apple2015about,mutlu2020retrospective}.
%\om{JUAN: cite 1. Apple security release, 2. Our TCAD 2019 paper.}. %JGL-2020-10-27

Second, an intelligent memory controller can greatly alleviate the
refresh problem in DRAM, and hence its negative consequences on
energy, performance, predictability, and technology scaling, by
understanding the retention time characteristics of different rows
well. It is well known that the retention time of different cells in
DRAM are widely different due to process manufacturing
variation~\cite{raidr,liu.isca13}. A very large fraction of all DRAM cells are strong (i.e., they
can retain data for hundreds of seconds), whereas only a small fraction of DRAM cells are weak
(i.e., they can retain data for only \SI{64}{\milli\second}), as demonstrated in Figure~\ref{fig:dram-refresh}~\cite{raidr,liu.isca13}.
Yet, today's memory
controllers treat \sg{every cell} as equal and refresh all rows every \SI{64}{\milli\second},
which is the \sg{worst}-case retention time that is allowed. This
worst-case refresh rate leads to a large number of unnecessary
refreshes, and thus great energy waste and performance loss. Refresh
is also shown to be the key technology scaling limiter of
DRAM~\cite{kang.memoryforum14}, and as such refreshing all DRAM cells
at the worst case rates is likely to make DRAM technology scaling
difficult.  An intelligent memory controller can overcome the refresh
problem by 1) identifying the minimum data retention time of each row
(during online operation) and 2) refreshing each row at the rate it
really requires to be refreshed at or 3) by \sg{decommissioning} weak rows
such that data is not stored in them. As shown by a recent body of
work whose aim is to design such an intelligent memory controller that
can perform online profiling of DRAM cell retention times and online
adjustment of refresh rate on a per-row
basis~\cite{raidr,liu.isca13,khan.sigmetrics14,qureshi.dsn15,khan.dsn16,khan.cal16,patel2017reaper,khan.micro17},
including the works on RAIDR~\cite{raidr,liu.isca13},
AVATAR~\cite{qureshi.dsn15} and REAPER~\cite{patel2017reaper}, such an
intelligent memory controller can eliminate more than 75\% of all
refreshes at very low cost, leading to significant energy reduction,
performance improvement, and quality of service benefits, all at the
same time, at the system level. Thus, the downsides of DRAM refresh can potentially be
overcome with the design of intelligent memory controllers.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/dram-refresh.pdf}
\vspace{-5mm}
\caption{Data retention times of different DRAM cells, represented as a cartoon based on experimental data obtained from real DRAM chips~\cite{kim2009new}.
%\om{JUAN: Please cite Samsung's EDL 2009 paper that is cited in our RAIDR paper}. 
Reproduced from~\cite{mutlu.nsfpim20}. Originally presented in~\cite{raidr.isca2012talk,mutlu.isca2013talk}.
%\om{JUAN: CITE Jamie's ISCA 2012 and my ISCA 2013 presentations.}
}
\label{fig:dram-refresh}
\end{figure}



%%% New Paragraph 1 
%%% @@@ONUR: Talk about the need for intelligent control for
%%% performance improvement: latency reduction and voltage reduction
%%% and subarray parallelism, etc: TL-DRAM, AL-DRAM, FLY-DRAM, DIVA
%%% DRAM, Solar-DRAM, SALP, Voltron
\sg{Third, an intelligent memory controller can enable performance
  improvements that can overcome the limitations of memory scaling.
  As we discuss in Section~\ref{sec:majortrends}, DRAM latency has
  remained almost constant over the last decades, despite the
  fact that low-latency computing has become even more important during
  that time. Similar to how intelligent memory controllers handle the
  refresh problem, the controllers can exploit the fact that not all
  cells in DRAM need the same amount of time to be accessed.
  Modern DRAM specifications require worst-case timing parameters that define the amount of
  time required to perform a memory access.  In order to guarantee
  correct operation, the timing parameters are chosen to ensure that
  the \emph{worst-case} cell in any DRAM chip that is acceptable (to satisfy a yield rate) can still
  be accessed correctly at \emph{worst-case operating
    temperatures}~\cite{chang.sigmetrics16, lee.hpca15,lee.sigmetrics17, kim2018solar,wang2018cal,hasan2019crow,luo2020clr}.
    %\om{JUAN: add more: 1. CAL-DRAM MICRO 2018, 2. CROW ISCA 2019, 3. CLR-DRAM ISCA 2020}. %jgl-2020-10-26
    However, we find that access
  latency to cells is very heterogeneous due to variation in 
  operating conditions (e.g., across different temperatures and
  operating voltage levels), manufacturing process (e.g., across different
  chips and different parts of a chip), and access patterns (e.g., based on
  whether or not the cell was recently accessed). We give eight examples
  of how an intelligent memory controller can exploit the various
  different types of heterogeneity in access latency.

  \sgii{(1)~At} low temperature, DRAM cells contain more charge, and
  as a result, can be accessed much faster than at high
  temperatures. We find that, averaged across 115 real DRAM modules
  from three major manufacturers, read and write latencies of DRAM can
  be reduced by 33\% and \sgii{55\%, respectively,} when operating at
  relatively low temperature (\sgii{\SI{55}{\celsius}}) compared to
  operating at worst-case temperature
  (\sgii{\SI{85}{\celsius}})~\cite{lee.hpca15, lee.thesis16}. Thus, a slightly
  intelligent memory controller can greatly reduce memory latency by
  adapting the access latency to operating temperature.

  \sgii{(2)~Due} to manufacturing process variation, we find that the
  majority of cells in DRAM (across different chips or within the same
  chip) can be accessed much faster than the manufacturer-provided
  timing parameters~\cite{chang.sigmetrics16, lee.hpca15,
    lee.sigmetrics17, kim2018solar, kevinchang-thesis, lee.thesis16}.  
  An intelligent memory controller
  can profile the DRAM chip and identify which cells can be accessed
  reliably at low latency, and use this information to reduce access
  latencies by as much as 57\%~\cite{chang.sigmetrics16,
    lee.sigmetrics17, kim2018solar}.

  \sgii{(3)~In} a similar fashion, an intelligent memory controller
  can use similar properties of manufacturing process variation to
  reduce the energy consumption of a computer system, by exploiting
  the minimum voltage required for safe operation of different parts
  of a DRAM chip~\cite{chang.sigmetrics17, kevinchang-thesis}. 
  The key idea is to reduce
  the operating voltage of a DRAM chip from the standard specification
  and tolerate the resulting errors by increasing access latency on a
  per-bank basis, while keeping performance degradation in check.

  \sgii{(4)~Bank} conflict latencies can be dramatically reduced by
  making modifications in the DRAM chip such that different subarrays
  in a bank can be accessed mostly independently\sgii{,} and designing
  an intelligent memory controller that can take \sgii{advantage} of
  requests that require data from different subarrays (i.e., exploit
  subarray-level parallelism)~\cite{salp, yoongu-thesis}. A similar approach is also shown to reduce the performance impact of refresh by enabling parallelization of refresh and access operations to a bank~\cite{chang.hpca14}.
  %\om{JUAN: Please cite Kevin chang's HPCA 2014 paper}. %JGL-2020-10-26

  \sgii{(5)~Access} latency to a portion of the DRAM bank can be
  greatly reduced by partitioning the DRAM array such that a subset of
  rows can be accessed much faster than the other rows and having an
  intelligent memory controller that decides what data should be
  placed in fast rows versus slow rows~\cite{lee.hpca13, lee.thesis16,luo2020clr,hasan2019crow,chang.hpca16,wang2020figaro}.
  %\om{JUAN: Also cite: 1. CLR-DRAM, 2, CROW, 3. LISA HPCA 2016, 4. FIGARO.}. %JGL-2020-10-26

  \sgii{(6)~We} find that a \sgii{recently-accessed or
    recently-refreshed} memory row can be accessed much more quickly
  than the standard latency if it needs to be accessed again soon,
  since the recent access and refresh to the row has replenished the
  charge of the cells in the row. An intelligent memory controller can
  thus keep track of the charge level of recently-accessed/refreshed
  rows and use the appropriate access latency that corresponds to the
  stored charge level~\cite{chargecache,wang2018cal,das.dac18}, leading to
  significant reductions in both access and refresh latencies.
  \sgii{Thus,} the poor scaling of DRAM latency and energy can
  potentially be overcome with the design of intelligent memory
  controllers that can facilitate a large number of effective latency
  and energy reduction techniques.}
  
  (7)~Two recent works~\cite{kim.hpca18,kim.hpca19} observe that the latency-reliability tradeoff in modern DRAM devices can be exploited by an intelligent memory controller to 1) generate true random numbers at low latency and high throughput~\cite{kim.hpca19}, and 2) to evaluate physical unclonable functions quickly using a DRAM device~\cite{kim.hpca18}. These works exploit the heterogeneity in the latency-reliability tradeoff of different cells: some cells fail truly randomly and some cells fail very consistently, when accessed with a low latency that violates the timing parameters. The former type of cells are used as true random number generator cells and the latter type of cells can be used as part of the challenge-response space of a DRAM-based physical unclonable function (PUF). An intelligent controller would determine the different types of cells using profiling mechanisms and enable the generation of true random numbers or PUF responses.
  
  (8)~An intelligent controller can use application and data characteristics to carefully map data across hybrid memories that consist of multiple different types of memories with different characteristics to maximize the benefits obtained from each memory type while avoiding the downsides of each memory type.
  Figure~\ref{fig:hybrid} depicts an example of such hybrid main memory composed of DRAM and PCM memories, as described by several works~\cite{meza2012enabling,yoon2012row,li2017utility,qureshi.isca09}.
  %\om{JUAN: Please cite 1. our ICCD 2012 RBLA paper, 2. Meza CAL 2012, 3. Our CLUSTER 2017 paper, 4. Moin's ISCA 2009 paper}.
  
  %\om{JUAN: Please see my comment about figure colors and screenshot I see in email.}

%JGL: I divided the paragraph to place the figure next to where it is referenced.
\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/hybrid-memory2.pdf}
\vspace{-5mm}
\caption{Hybrid main memory. Reproduced from~\cite{mutlu.iccdtalk19}. Originally presented in~\cite{yoon2012row}.
%\om{JUAN: CIte our RBLA ICCD 2012 paper.}
}
\label{fig:hybrid}
\end{figure}

  Many proposals exist for such intelligent controllers that manage hybrid memories, e.g.,~\cite{luo2014characterizing,ramos2011page,yu2017banshee,meza2012enabling,li2017utility,yoon2012row,qureshi.isca09,zhang2009exploring,song2020improving},
  %\om{JUAN: Please cite DATACON from ISMM 2020: "Improving Phase Change Memory Performance with Data Content Aware Access"} %JGL-2020-10-31
  %\om{JUan: Please cite 1. RBLA, ICCD 2012, 2. our CLUSTER 2017 paper, 3. Our HRM paper at dsn 2014, 4. Meza IEEE CAL 2012, 5. Banshee MICRO 2017, 6. Ramos ICS 2011, 7. and some more... please check the CLUSTER 2017 paper for more references}, %JGL-2020-10-27
  indicating that such an intelligent controller can enhance memory scaling by enabling the best of multiple technologies. For example, the idea of {\em Heterogeneous Reliability Memory}~\cite{luo2014characterizing} 
  %\om{JUAN: DSN 2014} %JGL-2020-10-26
  uses an intelligent memory controller that can communicate with both applications and memory devices to map each data element to different types of memories depending on the error vulnerability characteristics of the data element, thereby reducing memory cost. Similarly, EDEN~\cite{koppula2019eden} 
  %\om{JUAN: EDEN MICRO 2019} %JGL-2020-10-26
  uses a memory controller that can communicate with a neural network application to map different neural network layers to different DRAM partitions with different access latency and voltage parameters, depending on the error tolerance characteristics of each layer, thereby greatly improving energy efficiency and performance of neural network inference tasks. With increasing reliance on hybrid memories as well as increasing heterogeneity within each memory type to solve key memory scaling issues, it has become necessary to have intelligent controllers to manage data allocation, migration, and movement across the different heterogeneous parts. 
  
  %\om{ONUR TODO: Maybe talk about DRAM-PCM controllers specifically. Not sure yet.. + Pure pCM controllers like Hanbin's TACO 2014 work?}  


%%% New Paragraph 2
%%% ONUR:Talk about flash controllers already doing this... And, DRAM needing this soon as well. Basically, flash controllers are intelligent and they manage many things to make flash reliable, high performance, lower latency, etc etc. It is time DRAM controllers adopt a similar approach.

Intelligent controllers are already in widespread use in another key part of a modern computing system.  In solid-state drives (SSDs) consisting of NAND flash memory, the flash memory controllers that manage the SSDs are designed to incorporate a significant level of intelligence in order to improve both performance and reliability~\cite{yucai.bookchapter18,cai.bookchapter18.arxiv, yucai-thesis,luo.thesis18,tavakkol.fast18,tavakkol.isca18,cai.procieee17,cai2012error,cai2012flash,cai2013program,cai2013threshold,cai2014neighbor,cai2015data,cai2015read,cai2017vulnerabilities,luo2018heatwatch,luo2018improving,luo2014characterizing,luo2015warm,luo2016enabling,cai2013error,kim2020evanesco}.
    %\om{JUAN: Please add all of Yu Cai's and Yixin's works here that are on my Publications site. Lois used these recently and can provide them.}.  %JGL-2020-10-27
    %\om{JUAN: Do we have our Intel Tech Journal 2013 article in the preceding reference block? Please doble check. Let's make sure we have all our flash papers here. Please also do it in the below reference block. Please also add Evanesco} %JGL-2020-11-02
Figure~\ref{fig:flashI} shows one of our real experimental infrastructures (from~\cite{cai2012flash}) used for the design and evaluation of intelligent flash memory controllers.


%JGL: I divided the paragraph to place the figure next to where it is referenced.
\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/flash-controllers-I.pdf}
\vspace{-5mm}
\caption{Example of an intelligent flash memory controllers. The figure depicts a picture of one of our real experimental infrastructures (from~\cite{cai2012flash}) used for the design and evaluation of intelligent flash memory controllers. Reproduced from~\cite{mutlu.iccdtalk19}.}
\label{fig:flashI}
\end{figure}


Modern flash controllers need to take into account a wide variety of issues such as remapping
data, performing wear leveling to mitigate the limited lifetime of
NAND flash memory devices, refreshing data based on the current
wearout of each NAND flash cell, optimizing voltage levels to
maximize memory lifetime, employing sophisticated error correction and recovery techniques to maximize lifetime and minimize error rates, and enforcing fairness across different
applications accessing the SSD.  Much of the complexity in flash
controllers is a result of mitigating issues related to the scaling
of NAND flash memory~\cite{yucai.bookchapter18,cai.bookchapter18.arxiv,yucai-thesis,luo.thesis18,cai.procieee17,cai2012error,cai2012flash,cai2013program,cai2013threshold,cai2014neighbor,cai2015data,cai2015read,cai2017vulnerabilities,luo2018heatwatch,luo2018improving,luo2014characterizing,luo2015warm,luo2016enabling,cai2013error,kim2020evanesco}.
  %\om[JUAN: Please cite as above; all of Yu Cai and Yixin's works.}}. %JGL-2020-10-27
A comprehensive review of scaling issues of NAND flash memory and related mitigation techniques can be found in~\cite{cai.procieee17} (Figure~\ref{fig:flashII}) and~\cite{yucai.bookchapter18,cai.bookchapter18.arxiv}.
We argue that in order to overcome scaling
issues in main memory (DRAM), the time has come for main memory controllers to
also incorporate significant intelligence. Yet, incorporating sophisticated intelligence in the DRAM controller is more challenging than doing so in a flash controller due to the much lower access latency and much higher access bandwidth of modern DRAM devices.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/flash-controllers-II.pdf}
\vspace{-5mm}
\caption{A comprehensive review article on scaling issues of NAND flash memory and related mitigation techniques~\cite{cai.procieee17} Reproduced from~\cite{mutlu.iccdtalk19}.}
\label{fig:flashII}
\end{figure}


%%% New Paragraph 3
%%% Conclude with summarizing/reiterating the need for intelligent memory controllers for enhancing technology scaling and DRAM properties. And, say that the intelligence can be expanded to perform computation in applications. Foreshadow Section 4.

\sg{As we describe above, introducing intelligence into the memory
  controller can help us overcome a number of key challenges in memory
  scaling.  In particular, a significant body of work has
  demonstrated that the key reliability, refresh\sgii{,} and latency/energy
  issues in memory can be mitigated effectively with an intelligent
  memory controller that intelligently and meticulously manages the many different characteristics of underlying memory chips, which may consist of different types of memory technology. As we discuss in Section~\ref{sec:processorcentric}, such
  intelligence can go even further, by enabling the memory controllers
  (and the broader memory system) to perform application computation
  in order to overcome the significant data movement bottleneck in
  modern and future computing systems.}





\section{Perils of Processor-Centric Design}
\label{sec:processorcentric}
%\addcontentsline{toc}{part}{Perils of Processor-Centric Design}

%\om{ONUR TODO: Revisit this section to make it flow better.}


As described earlier, a major reason for performance and energy degradation in modern computing systems is the large amount of \emph{data movement} present in the systems. Such data movement is a natural consequence of the {\em processor-centric} execution model and design paradigm~\cite{burks.1946}, which creates a dichotomy between computation and memory/storage. The processor-centric design paradigm separates computation capability and memory/storage capability into two completely-separate system components (i.e., the computing unit versus the memory/storage unit) that are connected by long and energy-hungry interconnects: processing is done only in the computing unit, while data {is} stored in a completely {separate} place. As a result, data has to continuously move back and forth between the memory/storage unit and {the computing unit (e.g., CPU cores or accelerators)}, for any computation to be performed.

In order to perform an operation on data that is stored within memory,
a costly process is invoked. First, the CPU {(or an
  accelerator)} must issue a request to the memory controller, which
in turn sends a series of commands across the off-chip bus to the DRAM
module. Second, the data is read from the DRAM module and returned to
the memory controller. Third, the data is placed in the CPU cache
{and registers}, where it is accessible by the CPU
cores. Finally, the CPU can operate (i.e., perform computation) on the
data. All these steps consume substantial time and energy in order to
bring the data into the CPU
chip~\cite{kestor.iiswc2013,pandiyan.iiswc2014,kanev.isca15,boroumand.asplos18}.

{In current computing systems, the CPU (or any accelerator) is the only system
  component that is able to perform computation on data. The rest of
  system components are devoted to only data storage (memory, caches,
  disks) and data movement (interconnects); they are incapable of
  performing computation.} As a result, current computing systems are
\emph{grossly imbalanced}, which leads to large amounts of energy
inefficiency and lost performance. As empirical evidence to the gross
imbalance caused by the processor-memory dichotomy in the design of
computing systems today, we have recently observed that more than 62\%
of the entire system energy consumed by four major commonly-used
mobile consumer workloads (including the Chrome browser, TensorFlow
machine learning inference engine, and the VP9 video encoder and
decoder)~\cite{boroumand.asplos18}. Thus, the fact that current
systems can perform computation only in the computing unit (CPU cores
and hardware accelerators) is causing significant waste in terms of
energy by necessitating data movement across the entire system.


At least five factors contribute to the performance loss and the
energy waste associated with data movement between processor and memory. 
We briefly describe these next, to demonstrate the sweeping negative impact of data movement in modern computing systems.

First, the width of the off-chip bus between the memory controller and
the main memory is narrow, due to pin count and \sgii{cost} constraints,
leading to relatively low bandwidth and high latency to/from main memory. This makes {it} difficult to send a large number of requests to memory in
parallel to enable higher levels of parallelism and to tolerate the long main memory latency. As a result, systems that require higher levels of concurrency and lower latency require much higher cost because they require wider processor-memory interconnects or more processor-memory channels, both of which lead to higher power consumption and higher hardware area overheads~\cite{ghose2019demystifying,ghose2018vampire,mutlu.superfri15}.
%\om{JUAN: Please cite: 1. Demystifying... Saugata+ SIGMETRICS 2019, 2. VAMPIRE, Saugata SIGMETRICS 2018, 3. Our SUPERFRI paper.} %JGL-2020-10-26

Second, current computing systems employ many sophisticated mechanisms to tolerate the data access from main memory. These mechanisms include complex multi-level cache
hierarchies with sophisticated insertion/promotion/eviction policies and sophisticated latency tolerance/hiding mechanisms (e.g.,
{sophisticated caching algorithms at many different caching
  levels,} multiple complex prefetching techniques, {high amounts
  of multithreading, complex and power-hungry out-of-order execution mechanisms}). These components, while sometimes effective
at improving performance, are costly in terms of both die area and
energy consumption, {as well as the additional latency required
  to access/manage them}. When these components are not effective at improving performance, they result in a net energy waste and latency overheads that hurt the very performance that they are designed to improve. These components significantly increase the complexity of the system. Hence, the architectural and microarchitectural
techniques used in modern systems to tolerate the consequences of the
dichotomy between processing unit and main memory, lead to significant
energy waste and additional system complexity. As such, we are in a vicious cycle in system design due to the processor-centric design paradigm: 1) data movement between the processor and memory already causes significant energy waste and latency; 2) to tolerate the latency of such data movement, existing systems employ many complex mechanisms whose effectiveness varies depending on the workloads; 3) these complex mechanisms in turn cause additional energy waste and latency overheads. The fundamental cause of this vicious cycle is the processor-centric execution model and design paradigm, and hence breaking out of this vicious cycle requires tackling this fundamental cause by changing the paradigm (to a data-centric one).

Third, the many caches employed in computing systems are not always effective or efficient. Much of the data brought into the caches is \emph{not} reused by the
CPU~\cite{qureshi.isca07,qureshi-hpca07,ahn.pei.isca15,ahn.tesseract.isca15,seshadri2012evicted},
%\om{JUAN: Please cite Tesseract and PEI, + Evicted Address Filter, PACT 2012}, %JGL-2020-10-27
resulting in a large waste of hardware area and memory bandwidth. For example, 1) random access to memory leads to poor locality, rendering caches almost completely ineffective, 2) strided access to memory where stride is greater than a cache block also renders caches ineffective, 3) even streaming access to memory where all elements in a cache block are used in a consecutive manner is inefficient to handle with large caches because the block is not reused again. There are many such access patterns in a wide variety of modern workloads~\cite{qureshi.isca07,qureshi-hpca07,ahn.tesseract.isca15,ahn.pei.isca15,seshadri2012evicted,ghose2019demystifying,khan2014improving,qureshi2006case,DBLP:journals/tc/MutluKP06,subramanian-micro2015} 
%\om{JUAN: 1. Tesseract, 2.PEI, 3, EAF, PACT 2012, + many more caching works} %JGL-2020-10-28
that render caches either very inefficient or unnecessary, exacerbating the energy waste due to data movement in processor-centric systems.

Fourth, many modern applications, such as graph
processing~\cite{ahn.tesseract.isca15,ahn.pei.isca15} and workloads that operate on sparse data structures, such as sparse linear algebra~\cite{kanellopoulos2019smash,sadi2019efficient} and sparse neural networks~\cite{gondimalla2019sparten,hegde2019extensor,zhu2019sparse}, 
%\om{JUAN: 1. SMASH, and some more references + ALSO, can you give examples of other workloads than graph + sparse workloads. Adding another category would be good.}, 
produce random memory access patterns. 
Figure~\ref{fig:apps-graph} shows the example of PageRank~\cite{page1999pagerank}, a graph processing algorithm with frequent random memory accesses and little amount of computation. 
With such random access patterns, not only the caches but also the main memory bus and the main memory itself are very inefficient, since only a small part of each memory row and cache line retrieved all the way from main memory is actually used by the CPU. Such random accesses are fundamentally difficult to prefetch, rendering prefetchers ineffective.
{This example demonstrates that modern memory hierarchies are not designed to work well for random memory access \sg{patterns} that are found in many modern workloads.}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/apps-graph.pdf}
\vspace{-5mm}
\caption{Random memory accesses in the PageRank graph processing algorithm~\cite{page1999pagerank}. Reproduced from~\cite{mutlu.nsfpim20}. Originally depicted in~\cite{ahn.tesseract.isca15,ahn.tesseract.isca15talk}.
%\om{JUAN: Cite our Tesseract paper and talk}.
}
\label{fig:apps-graph}
\end{figure}


Fifth, the processor (as well as accelerators) and the main memory are connected to each other via long, power-hungry interconnects. {These interconnects impose
  significant additional latency to every data access and represent a
  significant fraction of the energy spent on moving data to/from the
  DRAM memory.} In fact, off-chip interconnect latency and energy
consumption is a key limiter of performance and energy in modern
systems~\cite{lee.hpca13,donghyuk-ddma,seshadri2013rowclone,GS-DRAM,ahn.tesseract.isca15,boroumand.asplos18}, 
%\om{JUAN: Please add: 1. Tesseract, 2. Google Workloads}, %JGL-2020-10-26
as it greatly exacerbates the cost of data movement. Unfortunately, off-chip interconnect latency and energy are not scaling (i.e., reducing) well with the scaling of technology node generations, which mainly benefits logic~\cite{dennard1974design}. 
%\om{JUAN: Please cite Dennard's original scaling paper}. %JGL-2020-10-26


The increasing disparity between processing technology and
memory/communication technology has resulted in systems in which
communication (data movement) costs dominate computation costs in
terms of energy consumption. The energy consumption of a main memory
access is between two to three orders of magnitude the energy
consumption of an addition operation today.  
For example,~\cite{pandiyan.iiswc2014} reports that the energy consumption
of a memory access is $\sim115\times$ the energy consumption of an
addition operation. 
Similarly, Figure~\ref{fig:datamov-energy} shows that compares the energy consumed by a DRAM access is $\sim800\times$ the energy consumption of a double precision addition operation, based on data reported by~\cite{dally.2015}. 
As a result, data movement is empirically shown to account for 40\%~\cite{kestor.iiswc2013}, 35\%~\cite{pandiyan.iiswc2014}, and 62\%~\cite{boroumand.asplos18} of the total system energy in
scientific, mobile, and consumer applications, respectively.  This
energy waste due to data movement is a huge burden that greatly limits
the efficiency and performance of all modern computing platforms, from
datacenters with a restricted power budget to mobile devices with
limited {battery life}.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/datamov-vs-energy.pdf}
\vspace{-5mm}
\caption{Data movement versus computation energy.  The figure depicts the absolute amount of energy spent on various arithmetic and data movement operations, including a double-precision floating point addition and a single DRAM access. Reproduced from~\cite{mutlu.nsfpim20}, based on data reported in~\cite{dally.2015}.}
\label{fig:datamov-energy}
\end{figure}


Overcoming all the reasons that cause low performance and large energy
inefficiency (as well as high system design complexity) in current
computing systems first requires the realization that all of these reasons are caused by the processor-centric design paradigm employed by existing computing systems. As such, a fundamental solution to all of these reasons at the same time requires a paradigm shift~\cite{kuhn2012structure}. 
%\om{JUAN: Cite Thomas KUhn's book}. %JGL-2020-10-26
We believe that future computing architectures should become \emph{data-centric}: {they should (1) perform computation with} minimal data movement, and (2) {compute} where it makes sense (i.e., where
the data resides), as opposed to computing solely in the processor (i.e., CPU or accelerators). Thus, the traditional rigid dichotomy between the
computing units and the memory/communication units needs to be broken
and a new paradigm enabling computation where the data resides needs
to be invented and enabled. We refer to this general data-centric execution model and design paradigm as {\em Processing-in-Memory (PIM)}.





\section{Processing-in-Memory (PIM): Technology Enablers and Two Approaches}
\label{sec:pim}
%\addcontentsline{toc}{part}{Processing-in-Memory (PIM): Technology Enablers and Two Approaches}

%One way to avoid the pitfalls of {the predominant} processor-centric compute model is to perform \emph{processing-in-memory} (PIM).
%PIM architectures offload some of the computation into the memory subsystem itself, eliminating unnecessary data movement.

Large amounts of data movement is a major result of the
  predominant processor-centric design paradigm of modern
  computers. Eliminating unnecessary data movement between memory 
  and the processor is essential to make future computing architectures
  high performance, energy-efficient and sustainable. To this
  end, \emph{processing-in-memory} (PIM) equips the memory \sg{subsystem}
  with the ability to perform computation.

In this section, we first describe two new technology enablers for PIM: 1) the emergence of 3D-stacked memories, and 2) the use of byte-addressable memories. These two relatively new main memory technologies provide new opportunities that can make it easier for modern computing systems to introduce and adopt PIM. 

Second, we introduce two promising approaches to implementing
PIM in modern architectures.  The first approach, {\em processing using memory}, exploits the existing
DRAM architecture and the operational principles of the DRAM circuitry
to enable (bulk) processing operations within the main memory with
minimal changes. This minimalist approach can especially be powerful
in performing specialized computation in main memory by taking
advantage of what the main memory substrate is extremely good at
performing with minimal changes to the existing memory chips.  The
second approach, {\em processing near memory}, exploits the ability to implement a wide variety of
general-purpose processing logic in the logic layer of 3D-stacked
memory and thus the high internal bandwidth {and low latency}
available {between the logic layer and the memory layers of}
3D-stacked memory. This is a more general approach where the logic
implemented in the logic layer can be general purpose and thus can
benefit a wide variety of applications. 

Below, we provide  a more detailed general overview of the two approaches, to show that the approaches are more general than what we will describe in more detail. It is important for the reader to keep in mind that the two approaches can be applied to many different types of memory technologies, even though our major focus will be on DRAM, the predominant main memory technology for several decades, in most of this section. 

%\jgl{Because processing-near-memory is a more obvious approach than processing-using-memory, I would suggest placing processing-near-memory first.}
%\om{I do not understand why PnM is more obvious. It all depends on your mindset and what you know. Better not to perpetuate old mindsets, if that is the reason why PnM is more "obvious". I would still like to keep the structure of my keynote talks and lectures.}

\subsection{New Technology Enablers: 3D-Stacked Memory and Non-Volatile Memory}
\label{sec:tech-enablers}
%\addcontentsline{toc}{part}{New Technology Enablers: 3D-Stacked Memory and Non-Volatile Memory}

Memory manufacturers are actively developing  new approaches for main memory system design, due to the DRAM technology scaling issues we described in detail in Section~\ref{sec:majortrends}. Two promising technologies are 3D-stacked memory and byte-addressable Non-volatile Memory (NVM), both of which can be exploited to overcome prior barriers to introducing and implementing PIM architectures.

\subsubsection{3D-Stacked Memory Architectures}
%\om{JUAN: Please add the citations to the below paragraphs from our IBM JRD paper + more citations as we would like...} %JGL-2020-10-28
The first major new approach to main memory design is 3D-stacked memory~\cite{ahn.tesseract.isca15,jedec.hbm.spec,lee.taco16,loh2008stacked,hmc.spec.1.1,hmc.spec.2.0}. %[5, 37-40]}. 
In a 3D-stacked memory, multiple layers of memory (typically DRAM in already-existing systems) are stacked on top of each other, as shown in Figure~\ref{fig:3d-dram}.
%\om{JUAN: Please add the figure from our IBM JRD paper's arxiv version. In caption, say "Reproduced from [X]." where [X] is our arxiv version of the JRD paper. } %JGL-2020-1-28
These layers are connected together using vertical through-silicon vias (TSVs)~\cite{loh2008stacked,lee.taco16}. %[38, 39]}. 
Using current manufacturing process technologies, thousands of TSVs can be placed within a single 3D-stacked memory chip. As such, the TSVs provide much greater internal memory bandwidth than the narrow memory channel. Examples of 3D-stacked DRAM available commercially include High-Bandwidth Memory (HBM)~\cite{jedec.hbm.spec,lee.taco16}, %[37, 38], 
Wide I/O~\cite{wideio}, %[115], 
Wide I/O 2~\cite{wideio2}, %[116], 
and the Hybrid Memory Cube (HMC)~\cite{hmc.spec.2.0}. %[40]. 
Detailed analysis of such 3D-stacked memories and their effects on modern workloads can be found in~\cite{lee.taco16,ghose2019demystifying,ramulator}.
%\om{JUAN: Please cite: 1. SMLA TACO 2016, 2. Saugata Demystifying SIGMETRICS 2019, 3. Ramulator CAL 2015.}. %JGL-2020-10-28

%\om{JUAN: Please insert Figure here. Please add the figure from our IBM JRD paper's arxiv version. In caption, say "Reproduced from [X]." where [X] is our arxiv version of the JRD paper.}
\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/3d-stacked-dram.pdf}
\vspace{-5mm}
\caption{High-level overview of a 3D-stacked DRAM architecture. Reproduced from~\cite{ghose2019arxiv}.}
\label{fig:3d-dram}
\end{figure}


In addition to the multiple layers of DRAM, a number of prominent 3D-stacked DRAM architectures, including HBM and HMC, incorporate a logic layer inside the chip~\cite{lee.taco16,jedec.hbm.spec,hmc.spec.2.0}. %[37, 38, 40]}. 
The logic layer is typically the bottommost layer of the chip, and is connected to the same TSVs as the memory layers. The logic layer provides area inside the DRAM chip where architects can implement functionality that interacts with both the processor and the DRAM cells. Currently, manufacturers make limited use of the logic layer and there is significant amount of area the logic layer can provide. This presents a promising opportunity for architects to implement new PIM logic in the available area of the logic layer. We can potentially add a wide range of computational logic (e.g., general-purpose cores, accelerators, reconfigurable architectures, or a combination of all three types of logic) in the logic layer, as long as the added logic meets area, energy, and thermal dissipation constraints, which are important and potentially limiting constraints in 3D-stacked systems.

\subsubsection{Non-Volatile Memory (NVM) Architectures}
%\om{JUAN: Please add the citations to the below paragraphs from our IBM JRD paper + more citations as we would like...} %JGL-2020-10-28
The second major new approach to main memory design is the development of byte-addressable resistive nonvolatile memory (NVM). In order to circumvent DRAM scaling limitations, such as refresh due to charge loss, as much as possible, researchers and manufacturers have been developing new memory devices that can store data at much higher densities than the typical density available in existing DRAM manufacturing process technologies. Manufacturers are exploring at least three types of emerging NVMs to augment or replace DRAM: (1) phase-change memory (PCM)~\cite{lee-isca2009,lee.cacm10,lee.ieeemicro10,qureshi.isca09,wong.procieee10,yoon-taco2014,zhou.isca09}. %[50-56]}, 
(2) magnetic RAM (MRAM)~\cite{kultursay.ispass13,naeimi.itj13}, %[57, 58]}, 
and (3) metal-oxide resistive RAM (RRAM) or memristors~\cite{chua.tct71,strukov.nature08,wong.procieee12}. %[59-61]}. 
All three of these NVM types are expected to provide memory access latencies and energy usage that are competitive with or close enough to DRAM, while enabling much larger capacities per chip and nonvolatility in main memory.
Since they are emerging and their designs do not have the long-term "baggage" other main memories (DRAM) have accumulated, NVMs present architects with an opportunity to redesign how the main memory subsystem operates from the cell and chip levels all the way up to software and algorithms. While it can be relatively difficult to modify the design of DRAM arrays due to the delicacy of DRAM manufacturing process technologies as we approach scaling limitations, NVMs have yet to approach such scaling limitations. As a result, architects can potentially design NVM memory arrays that integrate PIM functionality from the getgo. A promising direction for this functionality is the ability to manipulate NVM cells at the circuit level in order to perform logic operations using the memory cells themselves. A number of recent works have demonstrated that NVM cells can be used to perform a complete family of Boolean logic operations~\cite{li.dac16,levy.microelec14,kvatinsky.tcasii14,angizi2018pima,angizi2018cmp,angizi2019dna}, %[41-46]}, 
similar to such operations that can be performed in DRAM cells~\cite{seshadri.micro17,seshadri.bookchapter17,Seshadri:2015:ANDOR,seshadri.arxiv16,seshadri2020indram}. %[18, 20, 47-49]}. 
NVMs have also been shown to perform more sophisticated operations like multiplication~\cite{ankit2019puma,shafiee2016isaac,chi2016prime}, %\om{JUAN: Please cite.}, 
which are more difficult to implement in DRAM.


\subsection{Two Approaches: Processing Using Memory (PUM) vs. Processing Near Memory (PNM)}
%\addcontentsline{toc}{part}{Two Approaches: Processing Using Memory (PUM) vs. Processing Near Memory (PNM)}

Many recent works take advantage of the memory technology innovations that we discuss in Section~\ref{sec:tech-enablers} to enable and implement PIM. We find that these works generally take one of two approaches, which are categorized in Table~\ref{tab:pum-pnm}: 
%\om{JUAN:Please fix table reference}: %JGL-2020-1028
(1) {\em processing using memory} or (2) {\em processing near memory}. We briefly describe each approach here. Sections~\ref{sec:PUM} and~\ref{sec:PNM} will provide example approaches and more detail for both.

%\om{JUAN: Please add Table 1 from our JRD paper arxiv version, except place PuM on top.}
\begin{table}[h]
\caption{Summary of enabling technologies for the two approaches to PIM used by recent works. Adapted from~\cite{ghose2019arxiv}.}
%\vspace{-2mm}
\label{tab:pum-pnm}
%\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ll}
\toprule
\textbf{Approach} & \textbf{Enabling Technologies} \\
\midrule
\multirow{5}{*}{Processing Using Memory} & SRAM  \\
                                        & DRAM  \\
                                        & Phase-change memory (PCM)  \\
                                        & Magnetic RAM (MRAM)  \\
                                        & Resistive RAM (RRAM)/memristors  \\
\hline
\multirow{3}{*}{Processing Near Memory} & Logic layers in 3D-stacked memory  \\
                                        & Silicon interposers  \\
                                        & Logic in memory controllers  \\
\bottomrule
\end{tabular}
}
\end{table}


%\om{JUAN: Please add citations to below paragraphs from our JRD paper + more...} %JGL-2020-10-28
{\em \bf Processing using memory (PUM)} exploits the existing
memory architecture and the operational principles of the memory circuitry
to enable operations within main memory with
minimal changes. PUM makes use of intrinsic properties and operational principles of the memory cells and cell arrays themselves, by inducing interactions between cells such that the cells and/or cell arrays can perform useful computation. Prior works show that processing using memory is possible using static RAM (SRAM)~\cite{aga.hpca17,eckert2018neural,fujiki2019duality,kang.icassp14}, %[63, 76, 100]}, 
DRAM~\cite{chang.hpca16,seshadri.micro17,seshadri2013rowclone,seshadri2020indram,seshadri.bookchapter17.arxiv,seshadri.bookchapter17,seshadri.arxiv16,Seshadri:2015:ANDOR,angizi2019graphide}, %[17-20, 47-49, 80, 87, 118]}, 
PCM~\cite{li.dac16}, %[41]}, 
MRAM~\cite{angizi2018pima,angizi2018cmp,angizi2019dna}, %[44-46]}, 
or RRAM/memristive~\cite{levy.microelec14,kvatinsky.tcasii14,shafiee2016isaac,kvatinsky.iccd11,kvatinsky.tvlsi14,gaillardon2016plim,bhattacharjee2017revamp,hamdioui2015memristor,xie2015fast,hamdioui2017myth,yu2018memristive} %[42, 43, 88, 92-99]} 
devices. Processing using memory architectures enable a wide range of different functions, such as bulk as well as finer-grained data copy/initialization~\cite{chang.hpca16,seshadri2013rowclone,aga.hpca17,rezaei2020nom,wang2020figaro}, 
%[17, 19, 63]}\om{JUAN: Please cite our NoM CAL 2020 paper as well + LISA + FIGARO}, %JGL-2020-10-28
bulk bitwise operations (e.g., a complete set of Boolean logic operations)~\cite{seshadri.micro17,li.dac16,angizi2018pima,angizi2018cmp,angizi2019dna,Seshadri:2015:ANDOR,seshadri.arxiv16,seshadri2020indram,aga.hpca17,li.micro17,mutlu2020retrospective,mandelman.ibmjrd02,chang.sigmetrics16,xin2020elp2im,gao2020computedram}, %[18, 41, 44-49, 63, 80, 106-108, 118]}, 
and simple arithmetic operations (e.g., addition, multiplication, implication)~\cite{levy.microelec14,kvatinsky.tcasii14,aga.hpca17,kang.icassp14,li.micro17,shafiee2016isaac,eckert2018neural,fujiki2019duality,kvatinsky.iccd11,kvatinsky.tvlsi14,gaillardon2016plim,bhattacharjee2017revamp,hamdioui2015memristor,xie2015fast,hamdioui2017myth,yu2018memristive,deng.dac2018,angizi2019graphide}. %[42, 43, 63, 76, 80, 88, 92-100]}.

{\em \bf Processing near memory (PNM)} involves adding or integrating PIM logic (e.g., accelerators, simple processing cores, reconfigurable logic) close to or inside the memory (e.g.,~\cite{fernandez2020natsa,cali2020genasm,kim.bmc18,ahn.pei.isca15,ahn.tesseract.isca15,boroumand.asplos18,boroumand2019conda,boroumand2016pim,boroumand.arxiv17,singh2019napel,asghari-moghaddam.micro16,JAFAR,chi2016prime,farmahini2015nda,gao.pact15,DBLP:conf/hpca/GaoK16,gu.isca16,guo2014wondp,hashemi.isca16,cont-runahead,hassan.memsys15,hsieh.isca16,kim.isca16,kim.sc17,DBLP:conf/IEEEpact/LeeSK15,liu-spaa17,morad.taco15,nai2017graphpim,pattnaik.pact16,pugsley2014ndc,zhang.hpdc14,zhu2013accelerating,DBLP:conf/isca/AkinFH15,gao2017tetris,drumond2017mondrian,dai2018graphh,zhang2018graphp,huang2020heterogeneous,zhuo2019graphq})
%[5, 6, 16, 21-25, 62, 64-73, 75, 77, 79, 81, 83-87, 90, 91, 117])\om{JUAN:Please cite a lot more here.}). %JGL-2020-10-28
Many of these works place PIM logic inside the logic layer of 3D-stacked memories or at the memory controller, but recent advances in silicon interposers (in-package wires that connect directly to the through-silicon vias in a 3D-stacked chip)~\cite{jedec.hbm.spec,fernandez2020natsa,singh2020nero}
%\om{JUAN: Please cite interposers here...} %JGL-2020-10-28
also allow for separate logic chips to be placed in the same die package as a 3D-stacked memory while still taking advantage of the TSV bandwidth. 

Note that more functionality can be potentially integrated into a memory chip using PNM than using PUM, but both approaches can be combined to get even higher benefit from PIM. In Section~\ref{sec:PUM}, we provide a detailed overview of PUM within the commodity DRAM technology. In Section~\ref{sec:PNM}, we provide a detailed overview of PNM within the 3D-stacked DRAM technology. We note that the described approaches and techniques in Sections~\ref{sec:PUM} and~\ref{sec:PNM} are applicable to other types of technologies as well, with small modifications. 





\section{Processing Using Memory (PUM)}
\label{sec:PUM}
\label{sec:minimally}
%\addcontentsline{toc}{part}{Processing Using Memory (PUM)}

%\subsection{Approach I: Minimally Changing Memory Chips}
%\jgl{This is the processing-using-memory section.}

The PUM approach to processing-in-memory
{modifies existing DRAM architectures minimally to extend their
  functionality with computing capability.  This approach takes
  advantage of the existing interconnects in and analog operational
  behavior of conventional DRAM architectures (e.g., DDRx, LPDDRx,
  HBM), without the need for a dedicated logic layer or logic
  processing elements}, and {usually} with very low overheads.
Mechanisms that use {this approach} take advantage of the high
internal bandwidth available within {each} DRAM cell
array. There are a number of example PIM architectures that make use
of the PUM approach~\cite{seshadri.bookchapter17,seshadri2013rowclone,chang.hpca16,kevinchang-thesis,seshadri.thesis16,Seshadri:2015:ANDOR, seshadri.arxiv16, seshadri.micro17,seshadri2020indram}.
  %\om{juan: cite in-dram BB execution engine}. %JGL-2020-10-27
  In this
section, we first focus on two such {designs}: {RowClone,
  which enables in-DRAM bulk data movement
  operations~\cite{seshadri2013rowclone} and Ambit, which enables
  in-DRAM} bulk bitwise operations~\cite{Seshadri:2015:ANDOR,seshadri.arxiv16,seshadri.micro17,seshadri2020indram}.
  %\om{juan: cite in-dram BB execution engine}. %JGL-2020-10-27
  Then, we describe a low-cost
substrate that {performs} data reorganization for non-unit
strided access patterns~\cite{GS-DRAM}.


\subsection{RowClone}
\label{sec:rowclone}
%\addcontentsline{toc}{part}{RowClone}
%\jgl{Title: In-DRAM Data Movement and Reorganization}

Two important classes of bandwidth-intensive memory operations are
(1)~\emph{bulk data copy}, where a large quantity of data is copied
from one location in physical memory to another; and (2)~\emph{bulk
  data initialization}, where a large quantity of data is initialized
to a specific value. We refer to these two operations as \emph{bulk
  data movement operations}. Prior
research\ch{~\cite{os-hardware,arch-os, kanev.isca15}} has shown that
operating systems \ch{and data center workloads} spend a significant
portion of their time performing bulk data movement
operations. For example, a paper by Google shows that close to 5\% of the execution time in Google's data center workloads is spent on executing only two data movement function calls, {\em memset} and {\em memcopy}. Therefore, accelerating these operations will likely
improve system performance \sg{and energy} efficiency.

%%RA: Shall we add LISA here as it is an extension to RowClone? we already cited LISA in the next set of citation block.
We have developed a mechanism called
\emph{RowClone}~\cite{seshadri2013rowclone}, which takes advantage of
the fact that bulk data movement operations do \emph{not} require any
computation on the part of the processor.  RowClone exploits the
internal organization and operation of DRAM to perform bulk data
copy/initialization quickly and efficiently inside {a DRAM chip}.
A DRAM chip contains multiple banks, where the banks are connected
together and to external I/O circuitry by a shared internal bus. Each bank
is divided into multiple
\emph{subarrays}~\cite{salp,chang.hpca14,seshadri2013rowclone}.  Each
subarray contains {many} rows of DRAM cells, where each column of
DRAM cells is connected together across the multiple rows using
\emph{bitlines}.

RowClone consists of two mechanisms that take advantage of the
existing DRAM structure.  The first mechanism, Fast Parallel Mode,
copies {the data of a row inside a subarray to another row}
inside the same DRAM subarray by issuing back-to-back activate (i.e.,
row open) commands to the source and the destination row.
Figure~\ref{fig:rowclone} illustrates the two steps of RowClone's Fast Parallel Mode. The first step activates source row $A$, which enables the capture of the entire row's data in the row buffer. The second step activates destination row $B$, which enables the copying of the contents of the row buffer into row $B$. Thus, the back-to-back activate in the same subarray enables the copying of source row $A$ to destination row $B$ by using the row buffer as a temporary buffer for row $A$'s contents.
The second
mechanism, Pipelined Serial Mode, {can transfer an arbitrary
  number of bytes} from a row in one bank to another row in another bank using the shared internal bus
among banks in a DRAM chip.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/rowclone.pdf}
\vspace{-5mm}
\caption{RowClone Fast Parallel Mode. Reproduced from~\cite{mutlu.nsfpim20}.}
\label{fig:rowclone}
\end{figure}


RowClone significantly reduces the raw latency and energy consumption
of bulk data copy and initialization, leading to $11.6\times$ latency
reduction and $74.4\times$ energy reduction for a {4kB bulk page
  copy (using the Fast Parallel Mode)}, at very low cost (only 0.01\%
DRAM chip area overhead)~\cite{seshadri2013rowclone}. This reduction
directly translates to improvement in performance and energy
efficiency of systems running copy or initialization-intensive
workloads.  {Our MICRO 2013 paper~\cite{seshadri2013rowclone}
  shows that the performance of six copy/\sgii{initialization}-\sg{intensive}
  benchmarks (including {the} fork system call,
  Memcached~\cite{memcached} and a MySQL~\cite{mysql} database)
  improves between 4\% and 66\%. For the same six benchmarks, RowClone
  reduces the energy consumption between 15\% and 69\%.}
  
  %\om{JUAN: please add citations below}
  Recent works have improved upon the RowClone approach in various ways. First, Low-cost Interlinked Sub-Arrays (LISA)~\cite{chang.hpca16} 
  %\om{CITE} %JGL-2020-10-27
  provides mechanisms to enable the rapid transfer of data between one subarray to and adjacent subarray in the same bank, by enhancing the connectivity of subarrays using isolation transistors. LISA reduces inter-subarray copy latency by 9.2$\times$ and DRAM energy by 48$\times$, approaching the \textit{intra-subarray} latency and energy improvements of RowClone's Fast Parallel Mode. Second, FIGARO~\cite{wang2020figaro} improves upon LISA by enabling fine-grained (i.e., column granularity) data copy across subarrays within a bank using the shared global I/O structures of the bank as an intermediate location. This work shows significant benefit from FIGARO when its principles and techniques are used to build a highly-effective yet low-cost in-DRAM cache. Third, Network-on-Memory (NoM)~\cite{rezaei2020nom} improves the parallelism of bank-to-bank copy as well as bank read/write operations by providing more connectivity between different banks and chip I/O structures using the logic layer in 3D-stacked memory. Fifth, the ComputeDRAM work~\cite{gao2020computedram} shows that one can mimic the effect of RowClone's back-to-back activation mechanism in off-the-shelf DRAM chips by violating the timing parameters such that two wordlines in a subarray are activated back-to-back as in Rowclone. This work shows that such a version of RowClone can operate reliably in a variety of off-the-shelf DRAM chips tested using the SoftMC infrastructure~\cite{hassan2017softmc,softmc.github}. Sixth, the PINATUBO work~\cite{li.dac16} show that RowClone can effectively be performed in emerging resistive memory chips, including Phase Change Memory (PCM)~\cite{lee-isca2009,qureshi.isca09}.
  %\om{JUAN: please cite ben Lee's and Moin's PCM works}. %JGL-2020-10-27
  
  We believe that RowClone provides very low-cost specialized support for a critical and often-used operation: data copy and initialization. In latency-critical systems, such as virtual machines, modern software is written to, as much as possible, avoid large amounts of data copy exactly because data copy is expensive in modern systems (because it goes through the processor over a bandwidth-bottlenecked memory bus). Eliminating copies as much as possible complicates software design, making it less maintainable and readable. If RowClone is implemented in real chips, perhaps the need for avoiding data copies will greatly diminish due to the more-than-an-order-of-magnitude latency reduction of page copy, leading to easier-to-write and easier-to-maintain software. As such, we believe that an idea as simple as RowClone (and the work that builds on it) can have exciting and forward-looking implications on making both systems and software much faster, more efficient and overall better.



\subsection{Ambit}
\label{sec:ambit}
%\addcontentsline{toc}{part}{Ambit}

In addition to bulk data movement and initialization, many applications make use of
\emph{bulk bitwise operations}, i.e., bitwise operations on large bit
vectors~\cite{btt-knuth,hacker-delight}.  Examples of such
{applications} include bitmap
indices~\cite{bmide,bmidc,fastbit,bicompression} used in databases,  bitwise scan acceleration~\cite{bitweaving} in databases, accelerated document filtering for web search~\cite{bitfunnel}, DNA sequence
alignment~\cite{bitwise-alignment,xin.shd.bioinformatics15,alser.bioinformatics17,kim.bmc18,alser2020sneakysnake,cali2020genasm,alser2019shouji},
%\om{JUAN: Please add GRIM Filter, GenASM, Shouji, Sneakysnake here}, %JGL-2020-10-27
encryption algorithms~\cite{xor1,xor2,enc1}, graph
processing~\cite{li.dac16}, and
networking~\cite{hacker-delight}. Accelerating bulk bitwise operations
can {thus} significantly boost the performance and energy
efficiency of a wide range applications.

In order to avoid data movement bottlenecks when the system performs
these {bulk} bitwise operations, we have recently proposed a new
\textbf{A}ccelerator-in-\textbf{M}emory for bulk \textbf{Bit}wise
operations (Ambit)~\cite{Seshadri:2015:ANDOR, seshadri.arxiv16,
  seshadri.micro17}.  Unlike prior approaches, Ambit uses the analog
operation of existing DRAM technology to perform bulk bitwise
operations.  Ambit consists of two components.  The first component,
Ambit--AND--OR, implements a new operation called \emph{triple-row
  activation}, where the memory controller simultaneously activates
three rows.  Triple-row activation, depicted in Figure~\ref{fig:ambit-tra}, performs a bitwise majority
function across the cells in the three rows, {due to the charge
sharing principles that govern the operation of the DRAM array}. 
In the initial state, all three rows are closed \circled{1}. In the example of Figure~\ref{fig:ambit-tra}, two cells are in the charged state. When the three wordlines are raised simultaneously \circled{2}, charge sharing results in a positive deviation of the bitline. After sense amplification \circled{3}, the sense amplifier drives the bitline to $V_{DD}$, and as a result, fully charges the three cells. 
By controlling the initial value of one of the three rows (e.g., $C$), we can use triple-row activation to perform a bitwise AND or OR of the other two rows, 
since the bitwise majority function can be expressed as $C(A+B)+\bar{C}(AB)$. 
The second component, Ambit--NOT, takes advantage of the two
inverters that are part of each sense amplifier in a DRAM
subarray. {Ambit--NOT exploits the fact that, at the end of the
sense amplification process, the voltage level of one of the
inverters represents the negated logical value of the cell.  The
Ambit design adds a special row to the DRAM array, which is used to
capture the negated value that is present in the sense amplifiers.
One possible implementation of the special
row~\cite{seshadri.micro17} is a row of \emph{dual-contact cells} (a 2-transistor 1-capacitor cell~\cite{2t-1c-1,migration-cell}) that connect to both inverters inside the sense amplifier.}  With the ability to perform AND, OR, and NOT operations, Ambit {is
functionally complete: It} can reliably perform \emph{any} bulk
bitwise operation completely using DRAM technology, even in the
presence of significant process variation
{(see \cite{seshadri.micro17} for details)}.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/ambit-tra.pdf}
\vspace{-5mm}
\caption{Triple-row activation in Ambit. Reproduced from~\cite{seshadri.micro17}.}
\label{fig:ambit-tra}
\end{figure}

Averaged across seven commonly-used bitwise operations ({\em not, and, or, nand, nor, xor, xnor}), Ambit with 8
DRAM banks improves bulk bitwise operation throughput by 44$\times$
compared to an Intel Skylake processor~\cite{intel-skylake}, and
32$\times$ compared to the NVIDIA GTX 745 GPU~\cite{gtx745}. Compared
to the DDR3 {standard}, Ambit reduces energy consumption of these
operations by 35$\times$ on average. Compared to HMC
2.0~\cite{hmc.spec.2.0}, Ambit improves bulk bitwise operation
throughput by 2.4$\times$. When integrated directly into the HMC 2.0
device, Ambit improves throughput by 9.7$\times$ compared to
processing in the logic layer of HMC 2.0.

The Ambit work also shows that porting bitmap-index based databases as well as the BitWeaving database to execute Ambit can greatly improve query latencies. For example, Ambit reduces the end-to-end query latencies  by 5.4$\times$ to 6.6$\times$ for bitmap-based databases, with larger improvements coming from cases where more data needs to be scanned in the database. For the BitWeaving database, which is specifically designed to maximize bitwise operations so that the database can be relatively easily accelerated on modern GPUs, Ambit reduces the end-to-end query latencies by 4$\times$ to 12$\times$, again with larger improvements coming from cases where more data needs to be scanned in the database. These results are clearly very promising on two important data-intensive applications. 

%\om{JUAN: Please update this paragraph with references from the PUM approach from the Table and Section we added from the ibm jrd paper.} %JGL-2020-10-28
A number of Ambit-like bitwise operation substrates have been proposed in recent years, making use of emerging resistive memory technologies, e.g., \sgii{phase-change memory}
(PCM)~\cite{lee-isca2009,lee.ieeemicro10,lee.cacm10,zhou.isca09,qureshi.isca09,yoon-taco2014},
SRAM~\cite{aga.hpca17,kang.icassp14,eckert2018neural,fujiki2019duality},
%\om{JUAN: Please add}, 
or specialized computational DRAM~\cite{li.micro17,angizi2019dna,xin2020elp2im,gao2020computedram,angizi2019graphide}.
%\om{JUAN: Please add}. 
These substrates can perform bulk bitwise operations in a special DRAM array augmented
with computational circuitry~\cite{li.micro17,deng.dac2018} and in 
resistive memories~\cite{li.dac16} 
%\jgl{I cannot find this one: \om{JUAN: Also cite a DAC 2018 PCM paper from Pitt}\om{This is it: Quan Deng, Lei Jiang, Youtao Zhang, Minxuan Zhang, Jun Yang: DrAcc: a DRAM based accelerator for accurate CNN inference. 168:1-168:6}} %JGL-2020-10-26: Citation was above -- deng.dac2018.
like \sgii{PCM}.  Substrates similar to Ambit can perform simple arithmetic operations in SRAM~\cite{aga.hpca17, kang.icassp14} and arithmetic and logical operations in memristors~\cite{kvatinsky.tcasii14, kvatinsky.iccd11, kvatinsky.tvlsi14, shafiee2016isaac, levy.microelec14}. All of these works have shown significant benefits from performing bitwise operations using memory, for a wide variety of applications, including databases, machine learning, graph processing, genome analysis, and using a variety of different memory technologies, including DRAM, SRAM, PCM, memristors. 

Recently, the ComputeDRAM work~\cite{gao2020computedram} showed that carefully violating timing parameters between activation commands can mimic the triple-row-activation operation of Ambit in some existing off-the-shelf DRAM chips, using the SoftMC infrastructure~\cite{hassan2017softmc}. Thus, in-DRAM AND and OR operations can be performed in some real off-the-shelf DRAM chips even though clearly such chips are not designed to perform such Ambit operations. This proof-of-concept demonstration shows that the ideas presented in Ambit may not be far from reality: if some existing DRAM chips that are not even designed for in-DRAM bulk bitwise operations can perform such operations, then DRAM chips that are carefully designed for such operations will hopefully be even more capable!
    
We believe it is extremely important to continue exploring such low-cost
Ambit-like \sgii{substrates,} as well as more sophisticated computational substrates\sgii{,}
for all types of memory technologies, old and new. Resistive memory
technologies are fundamentally non-volatile and amenable to in-place
updates, and as such, can lead to even less data movement compared
to DRAM, which fundamentally requires some data movement to sense, amplify and restore
the data. \sgii{Thus}, we believe it is very promising to examine the
design of both charge-based conventional and emerging resistive memory chips that can incorporate
Ambit-like bitwise \sgii{operations} and other types of suitable computation
capability. Going forward, it is also critical to research frameworks that can enable ease-of-programming of such substrates such that many algorithms can take advantage of the massive bit-level parallelism offered by Ambit-like PUM substrates. 


\subsection{Gather-Scatter DRAM}
\label{sec:gs-dram}
%\addcontentsline{toc}{part}{Gather-Scatter DRAM}

Many applications access data structures with different access
patterns {at different points in time}. Depending on the layout
of the data structures in the physical memory, some access patterns
require non-unit strides. As current memory systems are optimized to
access {sequential} cache lines, non-unit strided accesses
exhibit low spatial locality, {leading to memory bandwidth
  waste} and cache space waste.

Gather-Scatter DRAM (GS-DRAM)~\cite{GS-DRAM} is a low-cost substrate
that addresses this problem. It {performs} in-DRAM data structure
reorganization by accessing multiple values that belong to a strided
access pattern using a single read/write command {in the memory
  controller}. GS-DRAM uses two key new mechanisms.  First, GS-DRAM
remaps the data of each cache line to different DRAM chips such that
multiple values of a strided access pattern are mapped to different
chips. {This enables the possibility of gathering different
  parts of the strided access pattern concurrently from different
  DRAM chips.}  Figure~\ref{fig:gsdram} show an example mapping on four DRAM chips. Adjacent values and/or adjacent pairs of values are swapped.
  Second, instead of sending separate requests to each chip,
the GS-DRAM memory controller communicates a pattern ID to the memory
module, as Figure~\ref{fig:gsdram} shows. With the pattern ID, each DRAM chip computes the address to be
accessed independently via a custom \emph{column translation logic (CTL)} hardware that is part of the DRAM module. This way, the returned cache line contains
different values of the strided pattern gathered from different DRAM chips.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/gsdram2.pdf}
\vspace{-5mm}
\caption{GS-DRAM (Gather-Scatter DRAM) data mapping and chip control overview. CTL refers to Column Translation Logic hardware in the DRAM module. Reproduced from~\cite{GS-DRAM}.
%\om{JUAN: Figure quality seems low. Can we capture it better? Or maybe there is a presentation version of this that is better?}\jgl{I captured it in a different way. I hope it looks better. There is no similar figure in the presentation.}
}
\label{fig:gsdram}
\end{figure}


GS-DRAM achieves near-ideal memory bandwidth and cache utilization in
real-world workloads, such as in-memory databases and matrix
multiplication.  {For in-memory databases, GS-DRAM outperforms a
  transactional workload with column-store layout by $3\times$
  %\om{JUAN: Use this notation of times above when we report AMbit results as well.} %JGL-2020-10-27
  and an analytics workload with row-store layout by $2\times$, thereby
  providing the best performance \sg{for} both transactional and analytical
  queries on databases (which in general benefit from different types
  of data layouts).  For matrix multiplication, GS-DRAM is 10\% faster
  than the best-performing tiled implementation of \sg{the matrix
  multiplication algorithm}.} We note that the idea of GS-DRAM is completely independent of memory technology, and thus GS-DRAM can be used in any type of memory module, including DRAM, SRAM, PCM, memristors, STT-MRAM, RRAM. 

\subsection{In-DRAM Security Primitives}
\label{sec:puf-trng}
%\addcontentsline{toc}{part}{In-DRAM Security Primitives}

Secure computation is of critical importance in modern computing systems. Therefore, it is important for a PIM system to support fundamental security primitives that enable secure computation and security functions. Doing so would enable PIM systems to execute a wider range of workloads and do so securely. To this end, recent work shows that Processing Using Memory can provide two basic security primitives: by carefully violating DRAM access timing parameters and taking advantage of the resulting characteristics of different DRAM cells (i.e., whether they always/never fail or fail randomly), it is possible to use DRAM to generate Physical Unclonable Functions (PUFs)~\cite{kim.hpca18} and true random numbers (TRNs)~\cite{kim.hpca19}.

PUFs are commonly used in cryptography to identify devices based on the uniqueness of their physical microstructures. 
DRAM-based PUFs have two key advantages: (1) DRAM is present in many modern computing systems, and (2) DRAM has high capacity and thus can provide many unique identifiers. However, traditional DRAM PUFs exhibit unacceptably high latencies and are not runtime-accessible. Our recent work, the DRAM Latency PUF~\cite{kim.hpca18},  proposes a new class of fast, reliable DRAM PUFs that are runtime-accessible, i.e., that can be used during online operation with low latency. The key idea is to reduce DRAM read access latency below the reliable datasheet specifications using software-only system calls. Doing so results in error patterns
that reflect the compound effects of manufacturing variations
in various DRAM structures (e.g., capacitors, wires, sense amplifiers). Some DRAM cells fail always or not at all, and a combination of a set of such cells can be used to generate a unique identifier for the device. 
Figure~\ref{fig:dram-puf} illustrates the key idea of using the pattern of predictable access latency failures in a DRAM subarray to generate a unique DRAM device identifier.
An experimental characterization of 223 LPDDR4 DRAM chips from all three major manufacturers shows that these error patterns (1) satisfy runtime-accesible PUF requirements, and (2) are quickly generated (i.e., at 88.2ms) irrespective of operating
temperature. The DRAM latency PUF does not require any modification to existing DRAM chips -- it only requires an intelligent memory controller that can change timing parameters and identify DRAM regions and cells that can be reliably used as PUFs.

%\om{JUAN: I did not realize the slide was for retention failures. Let's use Slide 19 instead from DLPUF talk -- DLPUF Key idea slide} %https://people.inf.ethz.ch/omutlu/pub/dram-latency-puf_hpca18_talk.pdf}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/dram-puf2.pdf}
\vspace{-5mm}
\caption{Key idea of DRAM latency PUF. Reproduced from~\cite{kim.hpca18talk}.
%\om{JUAN: Replace figure and fix caption. Text should be OK in paragraph above.}
}
\label{fig:dram-puf}
\end{figure}


Intentionally violating DRAM access timing parameters can also be used to generate true random numbers inside DRAM. The technique we propose in~\cite{kim.hpca19} decreases the DRAM row activation latency (timing parameter tRCD) below the datasheet specifications to induce read errors, or activation failures. As a result, some DRAM cells, called TRNG (True Random Number Generator) cells, fail truly randomly. 
By aggregating the resulting data from multiple such TRNG cells, our technique, called D-RaNGe, provides a high-throughput and low-latency TRNG. Figure~\ref{fig:d-range} illustrates the key idea of D-RaNGe: finding and using the TRNG cells in a DRAM subarray to generate true random values.

We demonstrate the effectiveness of D-RaNGe in 282 LPDDR4 devices from the three major manufacturers, and observe that the produced random data remains robust over both time and temperature variation. D-RaNGe (1) successfully passes all NIST statistical tests for randomness, and (2) generates true random numbers with over two orders of magnitude higher throughput than the state-of-the-art DRAM-based TRNG. D-RaNGe does not require any modification to existing DRAM chips -- it only requires an intelligent memory controller that can change timing parameters and identify DRAM cells that can be reliably used as TRNG cells.


%\om{JUAN: Please use Slide 15 instead from the DRANGE talk - DRANGE Key Idea slide} 
%https://people.inf.ethz.ch/omutlu/pub/drange-dram-latency-based-true-random-number-generator_hpca19-talk.pdf for DRange}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/d-range.pdf}
\vspace{-5mm}
\caption{Key idea of D-RaNGe. Reproduced from~\cite{kim.hpca19talk}.
}
\label{fig:d-range}
\end{figure}


D-RaNGe and the DRAM Latency PUF show that commodity DRAM devices can be
reliably used to generate true random numbers and unique keys with
high throughput, low latency, and low power. As a result, PIM
systems can  effectively generate true random numbers and unique keys  directly using DRAM itself. Doing so can improve the security and privacy
of the system: PIM applications can  directly
generate random numbers or unique keys within DRAM
and do not require off-DRAM devices to generate them and
transfer them over the CPU to DRAM bus. Thus, random numbers or unique keys are no longer transferred across buses, and security-critical computations can securely happen inside memory, which likely vastly improves the security guarantees of a PIM-enabled system. 



\section{Processing Near Memory (PNM)}
\label{sec:PNM}
\label{sec:3dstacked}
%\addcontentsline{toc}{part}{Processing Near Memory (PNM)}

%\jgl{Should we incorporate other more recent works? GRIM-Filter, NATSA, GenASM?}\om{JUAN: Yes, can you add GRIM-filter from the IBM JRD paper + NATSA very briefly as separate subsections at the end of this Sec 7?} %JGL-2020-10-28

{\em Processing near memory (PNM)} involves adding or integrating PIM logic (e.g., accelerators, simple processing cores, reconfigurable logic) close to or inside the memory (e.g.,~\cite{fernandez2020natsa,cali2020genasm,kim.bmc18,ahn.pei.isca15,ahn.tesseract.isca15,boroumand.asplos18,boroumand2019conda,boroumand2016pim,boroumand.arxiv17,singh2019napel,asghari-moghaddam.micro16,JAFAR,chi2016prime,farmahini2015nda,gao.pact15,DBLP:conf/hpca/GaoK16,gu.isca16,guo2014wondp,hashemi.isca16,cont-runahead,hassan.memsys15,hsieh.isca16,kim.isca16,kim.sc17,DBLP:conf/IEEEpact/LeeSK15,liu-spaa17,morad.taco15,nai2017graphpim,pattnaik.pact16,pugsley2014ndc,zhang.hpdc14,zhu2013accelerating,DBLP:conf/isca/AkinFH15,gao2017tetris,drumond2017mondrian,dai2018graphh,zhang2018graphp,huang2020heterogeneous,zhuo2019graphq})
%[5, 6, 16, 21-25, 62, 64-73, 75, 77, 79, 81, 83-87, 90, 91, 117]\om{JUAN:Please cite a lot more here.}). %JGL-2020-10-28
Many of these works place PIM logic inside the logic layer of 3D-stacked memories~\cite{lee.taco16}.  This
\emph{PIM processing logic}, which we also refer to as \emph{PIM
  cores} or \emph{PIM engines}, interchangeably, can execute portions
of applications (from individual instructions to functions) or entire
{threads and applications,} depending on the design of the
architecture. Such PIM engines have high-bandwidth and low-latency
access to the memory stacks that \sg{are on} top of them, since the logic
layer and the memory layers are connected via high-bandwidth vertical
connections~\cite{lee.taco16}, e.g., through-silicon vias. In this
section, we discuss several examples of how systems can make use of relatively simple PIM
engines within the logic layer to avoid data movement and {thus
  obtain} significant performance and energy {improvements} on a
wide variety of application domains.

%\om{JUAN: Can we add a figure each for Tesseract and Ambit?}


\subsection{Tesseract: Coarse-Grained Application-Level PNM Acceleration of Graph Processing}
\label{sec:tesseract}
%\addcontentsline{toc}{part}{Tesseract: Coarse-Grained Application-Level PNM Acceleration of Graph Processing}

%\om{JUAN: For Tesseract, can you add Slide 113 in here: https://people.inf.ethz.ch/omutlu/pub/onur-NSF-PIM-KeynoteTalk-IntelligentArchitecturesForIntelligentMachines-October-26-2020-final.pdf ? The entire slide minus the page number and the SAFARI Logo is OK. Even SAFARI logo can stay...}  

A promising approach to using PNM is to enable coarse-grained acceleration of {\em entire applications} that are heavily memory bound. In such a fundamentally coarse-grained (i.e., application-granularity) approach, an entire application is re-written to completely execute on the PNM substrate, potentially using a specialized programming model and specialized architecture/hardware. This approach is especially promising because it can provide the maximum performance and energy benefits achievable from PNM acceleration of a given application, since it enables the customization of the entire PNM system for the application. We believe this approach can be especially promising for widely-used data-intensive applications, such as graph processing, machine learning, databases, media processing, genome analysis. 


A {popular modern} application is large-scale graph
processing~\cite{salihoglu.ssdbm13, tian.vldb13, low.vldb12,
  hong.asplos12, malewicz.sigmod10, harshvardhan.pact14,
  gonzalez.osdi12, ligra, Seraph, graphlab, nai2017graphpim}.
{Graph processing has} broad applicability and use in many
domains, from social {networks} to machine learning, from
{data analytics} to bioinformatics.  Graph analysis workloads
are known to put {significant} pressure on memory bandwidth due
to (1) large amounts of random memory accesses across large memory
regions (leading to very limited cache efficiency and very large
amounts of unnecessary data transfer on the memory bus) and (2) very
small amounts of computation per each data item {fetched from
  memory} (leading to very limited ability to hide long memory
latencies {and exacerbating the energy bottleneck by exercising
  the huge energy disparity between memory access and computation}).
These two characteristics make it very challenging to scale up such
workloads despite their inherent parallelism, especially with
conventional architectures based on large on-chip caches and
{relatively} scarce off-chip memory bandwidth {for random
  access}.

We can exploit the high bandwidth as well as \sg{the} potential computation
capability available within the logic layer of 3D-stacked memory to
overcome the limitations of conventional architectures for graph
processing.  To this end, we design a programmable PNM accelerator for
large-scale graph processing, called
Tesseract~\cite{ahn.tesseract.isca15}, depicted at a high level in Figure~\ref{fig:tesseract}.  Tesseract consists of (1) a
new hardware architecture that {effectively} utilizes the
available memory bandwidth in 3D-stacked memory by placing simple
in-order processing cores in the logic layer and enabling each core
\sg{to manipulate} data only on the memory partition it is assigned to
control, (2) an efficient method of communication between different
in-order cores within a 3D-stacked memory to enable each core to
request computation on data elements that reside in the memory
partition controlled by another core, and (3) a {message-passing
  based} programming interface, {similar to how modern
  distributed systems are programmed}, which enables remote function
calls on data that resides in each memory partition. The Tesseract
design moves functions (i.e., computations and temporary values) to data that is to be updated rather than moving data elements across
different memory partitions and cores. It also includes two hardware
prefetchers specialized for memory access patterns of graph
processing, which operate based on the hints provided by our
programming model.  Our comprehensive evaluations using five
state-of-the-art graph processing workloads with large real-world
graphs show that the proposed Tesseract PIM architecture improves
average system performance by {$13.8\times$} and achieves 87\%
average energy reduction over conventional systems.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/tesseract.pdf}
\vspace{-5mm}
\caption{Overview of the Tesseract system for graph processing. Reproduced from~\cite{mutlu.nsfpim20}. Originally presented in~\cite{ahn.tesseract.isca15,ahn.tesseract.isca15talk}.
%\om{JUAN: Please cite Junwhan's ISCA 2015 Tesseract talk as well}.
}
\label{fig:tesseract}
\end{figure}

A significant amount of recent research has built upon Tesseract to enable the graph processing PNM system to be much more powerful~\cite{dai2018graphh,zhang2018graphp,huang2020heterogeneous,zhuo2019graphq}. %These works include ...
Among these, GraphP~\cite{zhang2018graphp} proposes a new graph partitioning scheme that greatly reduces the costly communication across 3D-stacked memory chips. 
Better partitioning is also proposed in GraphH~\cite{dai2018graphh}, together with a reconfigurable double mesh network that provides higher bandwidth across 3D-stacked memory chips. 
GraphQ~\cite{zhuo2019graphq} employs static and structured communication patterns to eliminate irregular communication, which is one of the key bottlenecks of Tesseract. 
Hetraph~\cite{huang2020heterogeneous} combines memristor-based analog computation units and CMOS-based digital compute cores on the logic layer of 3D-stacked memory chips, in order to use the most suitable one for each phase of computation.
%\om{JUAN: Can you add 4-5 of the most revelant works, like GraphQ and very briefly say what they contribute + CITE}. %JGL-2020-10-28
Overall, combining the multiple proposals reported by these works, using the Tesseract-based PNM approach to accelerate graph processing can lead to more than two orders of magnitude improvement both in performance as well as energy efficiency compared to a conventional processor-centric system with high-bandwidth memory. This demonstrates the potential promise of designing an entire PNM system from the ground up completely for an important data-intensive application. 

%\jgl{Tesseract + references to followup works from others.}\om{JUAN: We should include key follow-up works from others at the end of the Tesseract section, i.e., in the above paragraph. Please address.}



\subsection{Function-Level PNM Acceleration of Mobile Consumer Workloads}
\label{sec:google}
%\addcontentsline{toc}{part}{Function-Level PNM Acceleration of Mobile Consumer Workloads}

Another promising approach to using PNM, {\em function-level offloading}, is less intrusive than Tesseract's application-granularity approach described in Section~\ref{sec:tesseract}. This approach can still be coarse-grained since the function that is offloaded to the PNM logic can be potentially arbitarily long. However, the entire application does not need to be re-written. This approach is promising because it can enable easier adoption of PNM while still providing significant benefits. The key question in this approach is which functions in an application should be offloaded for PNM acceleration. Several recent works tackle this question for various applications, e.g., mobile consumer workloads~\cite{boroumand.asplos18}, GPGPU workloads~\cite{pattnaik.pact16,hsieh.isca16},
%\om{JUAN: please cite TOM + Pattnaik et al.}, %JGL-2020-1027
graph processing and in-memory database workloads~\cite{boroumand2019conda,boroumand2016pim},
%\om{JUAN: please cite LazyPIM+CONDA}, %JGL-2020-1027
and a wide variety of workloads from many domains~\cite{oliveira2021pimbench}.
%\om{JUAN: cite our upcoming PIM WOrkloads paper} %JGL-2020-10-28
We will discuss function-level PNM acceleration of  mobile consumer workloads in this section, focusing on our recent work on the topic~\cite{boroumand.asplos18}.  

A very popular domain of computing today consists of consumer devices,
which include smartphones, tablets, web-based computers such as
Chromebooks, and wearable devices.  In consumer devices, energy
efficiency is a first-class concern due to the limited battery
capacity and {the stringent} thermal power budget.  We find that
\emph{data movement} is a major contributor to the total system energy
     {and execution time} in modern consumer devices.  Across all of
     the popular modern mobile consumer applications we study (described in the next
     paragraph), we find that 62.7\% of the total system
     energy, on average, is spent on data movement {across the
       memory hierarchy~\cite{boroumand.asplos18}.} As described before, this large fraction consumed on data movement is directly the result of the processor-centric design paradigm of modern computing systems.

We comprehensively analyze the energy and performance impact of data
movement for several widely-used Google consumer
workloads~\cite{boroumand.asplos18}, which account for a significant
portion of the applications executed on consumer devices.  These
workloads include (1)~{the Chrome web browser}~\cite{chrome}, which is
a very popular browser used in mobile devices and laptops;
(2)~{TensorFlow Mobile}~\cite{mobile-tensorflow}, Google's machine
  learning framework, which is used in services such as Google
  Translate, Google Now, and Google Photos; (3)~{the VP9 video
    playback engine}~\cite{vp9-specification}, and (4)~{the VP9
    video capture engine}~\cite{vp9-specification}, both of which are
  used in many video services such as YouTube and Google Hangouts.  We
  find that {offloading key functions to the logic layer} can
  greatly reduce data movement in all of these workloads.  However,
  there are challenges to introducing PIM in consumer devices, as
  consumer devices are extremely stringent in terms of the area and
  energy budget {they can accommodate for any new hardware
    enhancement}.  As a result, we need to identify what kind of
  in-memory logic can both (1)~\emph{maximize energy efficiency} and
  (2)~be implemented at \emph{minimum possible cost, in terms of both
    area overhead and complexity}.

We find that many of target functions for PIM in consumer workloads
are comprised of simple operations such as \emph{memcopy}, \emph{memset},
basic arithmetic and bitwise operations, {and simple data
  shuffling and reorganization routines}.  Therefore, we can
{relatively easily} implement these PIM target functions in
{the logic layer of 3D-stacked} memory using either (1)~a small
low-power general-purpose embedded core or (2)~a group of small
fixed-function accelerators.  Our analysis shows that the area of a
PIM core and a PIM accelerator take up no more than 9.4\% and 35.4\%,
respectively, of the area available for PIM logic in an
HMC-like~\cite{hmc.spec.2.0} 3D-stacked memory architecture.  Both the PIM
core and PIM accelerator eliminate a large amount of data movement,
and {thereby} significantly reduce total system energy (by an
average of 55.4\% across {all} the workloads) and execution time
(by an average of 54.2\%). 

As evident from these results, function-level acceleration provides significant performance and energy benefits, but the benefits are not as high as full application-level offloading and customization of the PNM system, as we have shown for Tesseract in Section~\ref{sec:tesseract}. This is expected since function-level offloading makes much fewer changes to the system and the programming model than application-level offloading, customization and rethinking of the system.  




\subsection{Programmer-Transparent Function-Level PNM Acceleration of GPU Applications}
\label{sec:gpu}
%\addcontentsline{toc}{part}{Programmer-Transparent Function-Level PNM Acceleration of GPU Applications}

In the last decade, Graphics Processing Units (GPUs) have become the
accelerator of choice for {a wide variety of} data-parallel
applications. They deploy thousands of in-order, {SIMT (Single
  Instruction Multiple Thread)} cores that run lightweight
threads. The heavily-multithreaded GPU architecture is devised to hide the long
latency of memory accesses by interleaving threads that execute
arithmetic and logic operations. Despite that, many GPU applications
are {still} very
%RA: Added ETC
\rachata{memory-bound~\cite{veynu.2011,jog.asplos2013,jog.isca2013,medic,nandita.2015,nandita.2016,jog.2016,mask,mosaic,rachata-thesis,li-asplos19},}
because the limited off-chip pin bandwidth cannot supply enough data
to the running threads.

Processing near memory in 3D-stacked memory architectures presents a promising opportunity to alleviate the memory bottleneck in GPU systems. GPU cores placed {in the logic layer of a 3D-stacked memory} can be directly
connected to the DRAM layers with high-bandwidth (and low-latency)
connections. 
Figure~\ref{fig:tom} presents an example configuration with a main GPU system connected to four 3D-stacked memories. In the logic layer of each 3D-stacked memory, there are GPU cores (also known as streaming multiprocessors, SMs) connected to memory vault controllers via a crossbar switch.
In order to leverage the potential performance benefits
of such systems, it is necessary to enable computation offloading and
data mapping to multiple {such compute-capable} 3D-stacked
memories, {such} that GPU applications can benefit from processing-in-memory capabilities in the logic layers {of such memories}.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/tom.pdf}
\vspace{-5mm}
\caption{Overview of a PNM GPU system with a powerful main GPU and less powerful logic-layer GPUs distributed across four 3D-stacked memories. Reproduced from~\cite{hsieh.isca16}.}
\label{fig:tom}
\end{figure}


TOM (Transparent Offloading and Mapping)~\cite{hsieh.isca16} proposes
two mechanisms to address computation offloading and data mapping
{in such a system} in a programmer-transparent manner.  First,
it introduces {new} compiler analysis {techniques} to
identify code sections in GPU kernels that can benefit from 
offloading to PIM engines. The compiler estimates the potential memory bandwidth
savings for each code block. To this end, {the compiler} compares
the bandwidth consumption of the code block, when executed on the
regular GPU cores, to the bandwidth cost of transmitting/receiving
input/output registers, when offloading to the GPU cores in the logic
layers. {At runtime, a final} offloading decision is made based
on dynamic system conditions, such as contention for processing resources in
the logic layer.  Second, a software/hardware {cooperative}
mechanism predicts the memory pages that will be accessed by offloaded
code, and places {such pages} in the same 3D-stacked memory 
where the code will be executed.  The goal is to make PIM effective by
ensuring that the data needed by the PIM cores is in the same memory
stack as the code that needs it.  {Both mechanisms are completely transparent to the
  programmer, who only needs to write regular GPU code without any
  explicit PIM instructions or any other modification to the code.}
We find that TOM improves the average performance {of a variety of GPGPU
  workloads} by 30\% and reduces the average energy consumption by
11\% with respect to a baseline GPU system without PIM offloading
capabilities.



A related work~\cite{pattnaik.pact16} identifies GPU kernels that are
suitable for PIM offloading by using a regression-based affinity
prediction model. A concurrent kernel management mechanism uses the
affinity prediction model and determines which kernels {should}
be scheduled concurrently {to maximize performance}. This way,
{the proposed} mechanism enables the simultaneous exploitation
of the regular GPU cores and the in-memory GPU cores. {This
  scheduling technique improves} performance and energy efficiency by
an average of 42\% and 27\%, respectively.

%\todo
%We have coupled PIM accelerators with GPUs using 3D-Stacked memories. The PIM accelerators are composed by GPU-like cores that are less powerful than the regular GPU cores because of the lower frequency and the absence of a cache hierarchy. Despite that, high speedups can be achieved due to the higher bandwidth and lower memory latency.
%We have explored different offloading granulities for these architectures. TOM detects candidates offloading candidates in runtime~\cite{hsieh.isca16}. These are sub-kernel blocks that are marked by the compiler and identified by the runtime. Another possibility is identifying the candidate at kernel boundaries~\cite{pattnaik.pact16}.




\subsection{Instruction-Level PNM Acceleration with PIM-Enabled Instructions (PEI)}
\label{sec:pei}
%\addcontentsline{toc}{part}{Instruction-Level PNM Acceleration with PIM-Enabled Instructions (PEI)}

%\om{JUAN: For PEI, can you add the uarch figure from our IBM JRD paper?}  

A finer-grained approach to using PNM is {\em instruction-level offloading}. With this approach, individual instructions can be offloaded to the PNM engine and accelerated. As we describe below, this fine-grained approach can have significant benefits in terms of potential adoption since existing processor-centric execution models already operate (i.e., perform computation) at the granularity of individual instructions and all such machinery can be reused to aid offloading to be as seamless as possible with existing programming models and system mechanisms. 
PIM-Enabled Instructions (PEI)~\cite{ahn.pei.isca15} aims to provide
the minimal processing-in-memory support to take advantage of PIM
using 3D-stacked memory, in a way that can achieve significant
performance and energy benefits without changing the computing system
significantly.  To this {end}, PEI proposes a collection of
simple instructions, which introduce small changes to the
computing system and no changes to the programming model or the
virtual memory system, in a system with 3D-stacked memory. These
instructions, generated by the compiler or programmer to indicate potentially PIM-offloadable operations in the program, are operations that can be executed either in a traditional host CPU (that fetches and decodes them) or the PIM engine in 3D-stacked memory.

PIM-Enabled Instructions are based on two key ideas. First, a PEI is a
cache-coherent, virtually-addressed host processor instruction that
operates on only a single cache block. It requires no changes to the
sequential execution and programming model, no changes to virtual
memory, minimal changes to cache coherence, and no need for special
data mapping to take advantage of PIM (because each PEI is restricted
to a single memory module due to the single cache block restriction it
has). Second, a Locality-Aware Execution runtime mechanism decides
dynamically where to execute a PEI (i.e., {either} the host
processor or the PIM logic) based on simple locality characteristics
and simple hardware predictors. {This runtime mechanism executes 
the PEI at the location that maximizes performance.}  In summary,
PIM-Enabled Instructions provide the illusion that PIM operations are
executed as if they were host instructions: the programmer may not even be aware that the code is executing on a PIM-capable system and the exact same program containing PEIs can be executed on conventional systems that do not implement PIM.

Figure~\ref{fig:pei} shows an example architecture that can be used to enable PEIs. In this architecture, a PEI is executed on a PEI Computation Unit (PCU). To enable PEI execution in either the host CPU or in memory, a PCU is added to each host CPU and to each vault in an HMC-like 3D-stacked memory. While the work done in a PCU for a PEI might have required multiple CPU instructions in the baseline CPU-only architecture, the CPU only needs to execute a single PEI instruction, which is sent to a central PEI Management Unit (PMU in Figure~\ref{fig:pei}). The PMU, which is in charge of the Locality-Aware Execution, launches the appropriate PEI operation on one of the PCUs, either on the CPU or in 3D-stacked memory. 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/pei.pdf}
\vspace{-5mm}
\caption{Example architecture for PIM-enabled instructions. Reproduced from~\cite{ghose2019arxiv}. Originally presented in~\cite{ahn.pei.isca15,ahn.pei.isca15talk}.
%\om{JUAN: Please cite and link to Junwhan's ISCA 2015 talk as well}.
}
\label{fig:pei}
\end{figure}


Examples of PEIs are integer increment, integer minimum,
floating-point addition, hash table probing, histogram bin index,
Euclidean distance, and dot product~\cite{ahn.pei.isca15}.
Data-intensive workloads such as graph processing, in-memory data
analytics, machine learning, and data mining can {significantly}
benefit from these PEIs.  Across 10 {key data-intensive}
workloads, we observe {that the use of PEIs in these workloads,
  in combination with the Locality-Aware Execution runtime mechanism,
  leads to an} average performance improvement of 47\% and an average
energy reduction of 25\% over a baseline \sg{CPU}, on reasonably large data set sizes. 

As such, the benefits provided by the fine-grained PEI approach are quite promising: with minimal changes to the system, performance and energy improve significantly. We therefore believe that the PEI mechanism can ease the adoption of PIM systems going into the future, a key issue we discuss in detail next. 


\subsection{Function-Level PNM Acceleration of Genome Analysis Workloads}
\label{sec:grim}
%\addcontentsline{toc}{part}{Function-Level PNM Acceleration of Genome Analysis Workloads}

Genome analysis is a critical data-intensive domain that can greatly benefit from acceleration~\cite{alser2020accelerating,mutlu.aacbbtalk19,alser.bioinformatics17,alser2019shouji,alser2020sneakysnake,xin.shd.bioinformatics15,cali2020genasm,cali2018nano,turakhia2018darwin,fujiki2018genax},
%\om{JUAN: Please cite our IEEE Micro survey and my AACBB keynote talk slides+video + ALSO CITE: 1. Gatekeeper, 2. Shouji, 3. SHD, 4. SneakySnake, 5. GenASM, 6. GenAX, 7. Darwin 8. Damla's BIB paper on Nanopore}, %JGL-2020-10-30
specifically processing-in-memory acceleration. We find that function-level PNM acceleration via algorithm-architecture co-design is especially beneficial for data-intensive genome analysis workloads, as demonstrated in two of our recent works~\cite{kim.bmc18,cali2020genasm}.
%\om{JUAN: Also cite GenASM}.

GRIM-Filter~\cite{kim.bmc18} is an in-memory accelerator for genome seed filtering. In order to read the genome (i.e., DNA sequence) of an organism, geneticists often need to reconstruct the genome from small segments of DNA known as reads, as current DNA extraction techniques are unable to extract the entire DNA sequence. A genome read mapper can perform the reconstruction by matching the reads against a reference genome, and a core part of read mapping is a computationally-expensive dynamic programming algorithm that aligns the reads to the reference genome. One technique to significantly improve the performance and efficiency of read mapping is seed filtering~\cite{xin.bmcgenomics13,xin.shd.bioinformatics15,alser2019shouji,alser.bioinformatics17,alser2020sneakysnake}, which reduces the number of reference genome seeds (i.e., segments) that a read must be checked against for alignment by quickly eliminating seeds with no probability of matching. GRIM-Filter proposes a state-of-the-art filtering algorithm, and places the entire algorithm inside memory~\cite{kim.bmc18}. 

GRIM-Filter represents the entire reference genome by dividing it into short continuous segments, called \emph{bins}, and performs analyses on metadata associated to each bin. This metadata, represented as a \emph{bitvector}, stores whether or not a particular \emph{token} (a short DNA sequence) is present in the associated bin. 
Bitvectors are stored in DRAM in column order, such that a DRAM access to a row fetches the bits of the same token across many bitvectors, as the left block of Figure~\ref{fig:grim} shows. GRIM-Filter places custom logic for each vault in the logic layer of 3D-stacked memory (center block of Figure~\ref{fig:grim}). In each vault, there are multiple \emph{per-bin logic modules} which operate on the bitvector of a single bin. Each logic module consists of an incrementer, accumulator, and comparator, as the right block of Figure~\ref{fig:grim} shows.
%This requires adding simple accelerators in the logic layer of 3D-stacked memory, and introducing 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/grim-filter.pdf}
\vspace{-5mm}
\caption{Left block: GRIM-Filter bitvector layout within a DRAM bank. Center block: 3D-stacked DRAM with tightly integrated logic layer stacked underneath with TSVs for high inter-layer data transfer bandwidth. Right block: Custom GRIM-Filter logic placed in the logic layer, for each vault. Reproduced from~\cite{kim.bmc18}.}
\label{fig:grim}
\end{figure}

GRIM-Filter introduces a communication protocol between the read mapper and the filter. The communication protocol allows GRIM-Filter to be integrated into a full genome read mapper (e.g., FastHASH~\cite{xin.bmcgenomics13}, mrFAST~\cite{alkan.naturegenetics09}, BWA-MEM~\cite{li2009fast}, Minimap2~\cite{li2018minimap2},
%\om{JUAN: Please cite}), 
by allowing (1) the read mapper to notify GRIM-Filter about the DRAM addresses on which to execute customized in-memory filtering operations, (2) GRIM-Filter to notify the read mapper once the filter generates a list of seeds for alignment. Across 10 real genome read sets, GRIM-Filter improves the performance of a full state-of-the-art read mapper by 3.65$\times$ over a conventional CPU-only system~\cite{kim.bmc18}.
%\om{JUAN: Let's use Fig 7 from the GRIM Filter paper. Can you incorporate here and in text?}


In a more recent work~\cite{cali2020genasm}, 
%\om{JUAN: GenASM}, 
we develop an algorithm-architecture co-design to accelerate {\em approximate string matching (ASM)}, which is used at multiple points during
the mapping process of genome analysis. ASM enables read mapping to account
for sequencing errors and genetic variations in the reads. Our work,
GenASM, is the first ASM acceleration framework
for genome sequence analysis. GenASM performs bitvector-based
ASM, which can efficiently accelerate multiple steps of
genome sequence analysis. We modify the underlying ASM
algorithm (Bitap~\cite{baeza1992new,wu1992fast}) 
%\om{JUAN: Let's cite bitap}) 
to significantly increase its parallelism and
reduce its memory footprint. We accelerate this modified ASM algorithm, called \emph{GenASM-DC} for Distance Calculation, using an accelerator that performs very efficient Distance Calculation between two input strings.
We also develop a novel Bitap-compatible algorithm for \emph{traceback} (i.e., a method to collect information about the different types of alignment errors, or differences, between two input strings), called \emph{GenASM-TB}. Using our modified algorithm and the new GenASM-TB algorithm, we design the first hardware accelerator for Bitap. 
Figure~\ref{fig:genasm} illustrates a high-level overview of GenASM, depicting the flow of input and intermediate data in the system as well as  the communication paths of the two accelerators for GenASM-DC and GenASM-TB.
Our hardware accelerator, which is placed in the logic layer of 3D-stacked memory to minimize data movement overheads, consists of specialized systolic-array-based compute units and on-chip SRAMs that are designed to match the rate of computation with memory capacity and bandwidth, resulting
in an efficient design whose performance scales linearly as we
increase the number of compute units working in parallel. Our detailed performance and energy evaluations demonstrate that GenASM provides significant performance
and power benefits for three different use cases in genome
sequence analysis, outperforming the best prior hardware accelerators as well as software baselines by one or more orders of magnitude. We believe these results are quite promising and point to the need for further exploration of PIM accelerators in genome analysis.

\begin{figure}[h]
\centering
%\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/bitap-TB-example.pdf}
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/genasm-pipeline.pdf}
\vspace{-5mm}
%\caption{Traceback example with GenASM-TB algorithm. Reproduced from~\cite{cali2020genasm}.}
\caption{Overview of GenASM. Different components are described in detail in~\cite{cali2020genasm}. Figure reproduced from~\cite{cali2020genasm}.}
\label{fig:genasm}
\end{figure}

%\om{JUAN: Let's include an overview figure for GenASM, but not explain it in detail. Can you add Fig 6 from the GenASM paper? I think that is very good. Please of course reference it from an appropriate point in the text above.}
%\om{JUAN: Sorry, I think I mistyped. I wanted Figure 4 (Overview of GenASM) not Fig 6. The Traceback figure is too dense for readers of this work to understand... Can you fix? -- I did keep your new explanation including and emphasizing TRaceback, though, so the effort was useful, just not the figure.}

\subsection{Application-Level PNM Acceleration of Time Series Analysis}
%\om{JUAN: NATSA is application-level, right?} %JGL: Yes, makes more sense.
\label{sec:natsa}
%\addcontentsline{toc}{part}{Application-Level PNM Acceleration of Time Series Analysis}

NATSA~\cite{fernandez2020natsa} is a near-memory processing accelerator for time series analysis. Time series analysis is a powerful technique for extracting and predicting events with applications in epidemiology, genomics, neuroscience, astronomy, environmental sciences, economics, etc. 
NATSA implements \emph{matrix profile}~\cite{yeh2016matrix}, the state-of-the-art algorithm for time series analysis fully via PNM. 
\emph{Matrix profile} operates on large amounts of time series data, but it has low arithmetic intensity. 
As a result, data movement represents a major performance bottleneck and energy waste, which NATSA alleviates by performing the complete time series analysis processing near memory using specialized accelerators. 
NATSA places energy-efficient floating point arithmetic processing units (PUs in Figure~\ref{fig:natsa}) close to 3D-stacked HBM memory~\cite{jedec.hbm.spec,lee.taco16}, 
%\om{JUAN: ALso cite SMLA TACO 2016}, 
connected via silicon interposers, 
as Figure~\ref{fig:natsa} shows.
NATSA improves performance by up to 14.2$\times$ (9.9$\times$ on average) and reduces energy by up to 27.2$\times$ (19.4$\times$ on average) over the state-of-the-art multi-core implementation. 
NATSA also improves performance by 6.3$\times$ and reduces energy by 10.2$\times$ over a general-purpose PNM platform with 64 in-order cores.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/NATSA_design_with_HBM.pdf}
\vspace{-5mm}
\caption{NATSA design and integration near HBM memory. A PU is a NATSA Processing Unit that can do energy-efficient floating point arithmetic for time series analysis. Its components are described in~\cite{fernandez2020natsa}. Figure reproduced from~\cite{fernandez2020natsa}.}
\label{fig:natsa}
\end{figure}



\section{Enabling the Adoption of PIM}
\label{sec:adoption}
%\addcontentsline{toc}{part}{Enabling the Adoption of PIM}

Pushing some or all of the computation for a program from the CPU to
{memory} introduces new challenges for system architects
{and programmers} to overcome.  
Figure~\ref{fig:pim-adoption} lists some of these key challenges. 
These challenges must be
addressed carefully and systematically in order for PIM to be adopted as a mainstream architecture
in a wide variety of systems and workloads, and in a seamless manner
that does not place heavy burden on the vast majority of programmers.
In this section, we discuss several of these system-level {and programming-level} challenges, and highlight a number of our works
that have addressed these challenges for a wide range of PIM
architectures. We believe future research should examine solutions to these challenges with an open mindset that is keen on enabling adoption, since the widespread success of the PIM paradigm critically depends on effective solutions to these challenges. 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/pim-adoption.pdf}
\vspace{-5mm}
\caption{Potential barriers to adoption of PIM. Reproduced from~\cite{mutlu.nsfpim20,mutlu.iccdtalk19}.}
\label{fig:pim-adoption}
\end{figure}


%\subsection{Code and Data Mapping}
\subsection{Programming Models and Code Generation for PIM}
\label{sec:mapping}
%\label{sec:pei}
%\addcontentsline{toc}{part}{Programming Models and Code Generation for PIM}

%\jgl{We can include programming of UPMEM. There are desirable programming features that are missing (libraries, portable programming and performance, high-level programming.}\om{Maybe after the SIGMETRICS paper is published, we can update this chapter at an appropriate place. I do not want this broad paper to consider specific issues with UPMEM.} 

%While processing-in-memory provides many opportunities to alleviate
%the main memory bottleneck, it is still challenging to integrate PIM
%architectures with existing systems in a seamless manner due
%to two common characteristics: unconventional programming
%models for in-memory computation units, and a lack of ability to
%utilize large on-chip caches.

%One approach to ease programming effort is to implement simple in-memory
%computation using compute-capable memory commands and
%use specialized instructions, which we call \emph{PIM-enabled instructions}~\cite{ahn.pei.isca15},  to invoke in-memory computation.   This allows
%PIM operations to be interoperable with existing programming models, cache coherence protocols, and virtual memory
%mechanisms with no modification. Our PIM-enabled instruction architecture provides the
%illusion that PIM operations are executed as if they were host
%processor instructions.

Two open research questions to enable the adoption of PIM are 1) what
should the programming {models} be, and 2) how can compilers and
libraries alleviate the programming burden?

While PIM-Enabled Instructions~\cite{ahn.pei.isca15} work well for
offloading fine-grained and small amounts of computation to memory, they can
potentially \chii{introduce overheads while taking} advantage of PIM
for large tasks, due to the need to frequently exchange information
between \chiii{the PIM processing logic} and the CPU.  Hence, there is
a need for researchers to investigate how to integrate PIM
instructions with other compiler-based methods or library calls that
can support PIM integration, and how these approaches can ease the
burden on the programmer, by enabling seamless offloading of
instructions or function/library calls.

Such solutions can often be platform-dependent.  One of our recent
works~\cite{hsieh.isca16} examines compiler-based mechanisms to decide
what portions of code should be offloaded to PIM processing logic in a
GPU-based system in a manner that is transparent to the GPU
programmer.  Another recent work~\cite{pattnaik.pact16} examines
system-level techniques that decide which GPU application kernels are
suitable for PIM execution.

As described in Section~\ref{sec:PNM} with multiple promising examples, different granularities of code offloading in Processing Near Memory architectures have different implications for performance and energy as well as system complexity. These different granularities also have implications on programming and code generation complexity. Adoption-minded solutions should clearly take into account the granularity of code offloading and how a PNM system supports code execution. 

Similarly, programming and code generation frameworks for Processing Using Memory approaches like Ambit are also critical for such approaches to become widely adopted. Programming model, compiler and library support for expressing, extracting and generating bulk bitwise operations in a program can greatly help the adoption of in-memory bulk bitwise execution models like Ambit. We believe there is exciting research to do in these directions.  

Determining {effective programming interfaces} and the necessary as well as useful compiler/library support to effectively perform PIM remain open research
{and design questions, which are important for future works to
  tackle.}



%\subsection{Scheduling}
\subsection{PIM Runtime: Scheduling and Data Mapping}
\label{sec:scheduling}
%\addcontentsline{toc}{part}{PIM Runtime: Scheduling and Data Mapping}

%\jgl{This could be divided into two sections. 
%Scheduling (what to execute in memory) can incorporate the list of conditions in Section 3.2 of the JRD paper. This list is preliminary and a more extensive analysis to understand conditions better is necessary (PIM benchmarks). 
%For data mapping, it would be good to mention the challenges in processing-using-mapping for achieving the appropriate mapping to be able to perform computation (e.g., alignment of data arrays); another challenge is the potential need for relocation in the middle of the execution: the NoM paper (CAL) would be good here.}
%\om{JUAN: I am fine with your suggestions. Can you add the suggested ideas without changing the other parts of the section? I like the idea of keeping the section as a single one for now -- you can use subsections.}

%\todo
%At least four key runtime issues in PIM are to decide (1)~when to enable PIM
%execution, (2)~what to execute near data, (3)~how to map data to multiple
%(hybrid) memory modules such that PIM execution is viable and effective, and
%(4)~how to effectively share/partition PIM mechanisms/accelerators at runtime
%across multiple threads/cores to maximize performance and energy efficiency.
%We will develop dynamic and adaptive mechanisms, both in software (OS, hypervisor
%and compiler) and hardware, to tackle all of these issues that are interrelated
%with each other. We will explore mechanisms to map data and schedule code with
%no or minimal programmer effort.  We will examine both static and adaptive data
%mapping mechanisms to intelligently map data that is operated on by the same
%code to the same memory stack. We will develop low-cost and low-overhead data
%migration mechanisms to facilitate easier PIM execution in case data mapping
%needs to be adapted to execution and access patterns at runtime. We will build

%It is possible to build on our recent works that employ locality
%prediction~\cite{ahn.pei.isca15} and combined compiler and dynamic code
%identification and scheduling in GPU-based systems~\cite{hsieh.isca16,pattnaik.pact16}. 

We identify four key runtime issues in PIM: (1)~what {code} to
execute near data, (2)~when to schedule execution on PIM (i.e., when
is it worth offloading computation to the PIM cores), (3)~how to map
data to multiple memory modules such that PIM execution is viable and
effective, and (4)~how to effectively share/partition PIM
mechanisms/accelerators at runtime across multiple threads/cores to
maximize performance and energy efficiency.  We have already proposed
several approaches to solve these four issues, yet much research remains to be done to enable a robust and effective PIM runtime system that can be effective under many conditions.

The first key issue is to identify which portions of an application are suitable for PIM. We call such portions \emph{PIM offloading candidates}. While PIM offloading candidates can be identified manually by a programmer, the identification would require significant programmer effort along with a detailed understanding of the hardware tradeoffs between CPU cores and PIM cores. For architects who are adding custom PIM logic (e.g., fixed-function accelerators, which we call PIM accelerators) to memory, the tradeoffs between CPU cores and PIM accelerators may not be known before determining which portions of the application are PIM offloading candidates, since the PIM accelerators are tailored for the PIM offloading candidates.
To alleviate the burden of manually identifying PIM offloading candidates, we develop a systematic toolflow for identifying PIM offloading candidates in an application~\cite{boroumand.asplos18,boroumand.arxiv17,boroumand2016pim,boroumand2019conda}. This toolflow uses a system that executes the entire application on the CPU to evaluate whether each PIM offloading candidate meets the constraints of the system under consideration. For example, when we evaluate workloads for mobile consumer devices (e.g., Chrome web browser, TensorFlow Mobile, video playback, and video capture)~\cite{boroumand.asplos18}, we use hardware performance counters and our energy model to identify candidate functions that could be PIM offloading candidates. A function is a PIM offloading candidate in a mobile consumer device if it meets the following conditions:
%\om{JUAN: I modified the first item below to be more general.}
\begin{enumerate}
\item It consumes a significant fraction (e.g., more than 30\%) of the overall workload energy consumption, since energy reduction is a primary objective in mobile systems and workloads.
\item Its data movement consumes a significant fraction (e.g., more than 30\%) of the total workload energy to maximize the potential energy benefits of offloading to PIM. 
\item It is memory-intensive (e.g., its last-level cache misses per kilo instruction, or MPKI, is greater than 10~\cite{chou2015reducing,kim2010atlas,muralidhara2011reducing,kim2010thread}), as the energy savings of PIM is higher when more data movement is eliminated.
\item Data movement is the single largest component of the function’s energy consumption.
\end{enumerate}
%JGL-2020-10-29
Figure~\ref{fig:google-methodology} shows two example functions in Google's Mobile TensorFlow machine learning inference framework~\cite{mobile-tensorflow,abadi2016tensorflow} 
%\om{JUAN: Please cite Tensorflow and Tensorflow mobile} %JGL-2020-11-02 
that are identified to be PIM offloading candidates using the afore-described methodology:  {\em packing/unpacking} and {\em quantization}~\cite{boroumand.asplos18}. Note that these functions are together responsible for more than 54\% of the data movement energy in the examined neural networks for this workload, which spend more than 57\% of their execution energy on data movement, as depicted in Figure~\ref{fig:google-methodology}.  

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/google-methodology.pdf}
\vspace{-5mm}
\caption{A majority of the data movement energy in TensorFlow Mobile machine learning inference framework~\cite{abadi2016tensorflow,mobile-tensorflow} 
%\om{JUAN: Please cite Tensorflow and Tensorflow mobile} 
is caused by two key functions. Reproduced from~\cite{mutlu.nsfpim20}. 
Originally presented in~\cite{boroumand.asplos18,boroumand.asplos18talk}.
%\om{JUAN: Please cite Amirali's ASPLOS 2018 talk as well}.
}
\label{fig:google-methodology}
\end{figure}




Some of our other recent works in PIM identify suitable %\emph{PIM offloading candidates} 
PIM offloading candidates 
with different granularities. PIM-Enabled
Instructions~\cite{ahn.pei.isca15} {propose various} operations
that can benefit from execution near or inside memory, such as integer
increment, integer minimum, floating-point addition, hash table
probing, histogram bin index, Euclidean distance, and dot product.
%In~\cite{boroumand.asplos18}, we find {simple} functions with
%intensive data movement that are suitable for PIM in consumer
%workloads (e.g., Chrome web browser, TensorFlow Mobile, video
%playback, and video capture), {as described in Section~\ref{sec:google}}. %JGL-2020-10-29
GPU applications also contain several parts that are suitable
{for offloading to PIM
  engines}~\cite{hsieh.isca16,pattnaik.pact16}.
%JGL-2020-11-06: I swapped the previous and the next sentence.
Bulk memory operations (copy,
\sg{initialization}) and {bulk} bitwise operations are good candidates
for Ambit-like processing using DRAM approaches~\cite{seshadri2013rowclone,seshadri.micro17,Seshadri:2015:ANDOR, seshadri.thesis16}, as we discussed earlier. 
For PUM approaches that can execute more complex operations (e.g., addition, multiplication) using memory, the \emph{operation complexity} (i.e., the latency of an operation for a certain data type) can determine how beneficial offloading to PUM can be compared to CPU execution. A recent analytical model~\cite{korgaonkar2019bitlet} helps to evaluate such offloading tradeoffs in memristor-based PUM~\cite{kvatinsky.tcasii14,kvatinsky.iccd11,kvatinsky.tvlsi14}.

In several of our research works, we propose runtime mechanisms for
\emph{dynamic scheduling} of PIM offloading candidates, i.e.,
mechanisms that decide whether or not to actually offload code that is
marked to be potentially offloaded to PIM engines.
In~\cite{ahn.pei.isca15}, we develop a locality-aware scheduling
mechanism {for PIM-enabled instructions}.  For GPU-based
systems~\cite{hsieh.isca16,pattnaik.pact16}, we explore the
combination of compile-time and runtime mechanisms for identification
and dynamic scheduling of PIM offloading candidates.

%\om{JUAN: I made some changes below for clarity.}
The best \emph{mapping of data and code} that enables the maximal
benefits from PIM depends on the applications and the computing system
configuration as well as the type of PIM employed in the system. 
For instance, in order to be able operate on two source arrays inside DRAM with PUM approaches~\cite{chang.hpca16,seshadri.micro17,seshadri2013rowclone,seshadri2020indram,seshadri.bookchapter17.arxiv,seshadri.bookchapter17,seshadri.arxiv16,Seshadri:2015:ANDOR,angizi2019graphide}, one key issue is how to guarantee the alignment of the two arrays inside the same DRAM subarray. Practical solutions for this issue need to involve both the memory controller and the operating system to enable that arrays aligned in virtual memory can also be physically aligned in DRAM. he programmer and/or the compiler also likely need to carefully annotate and communicate computation patterns on large data blocks so that the system software and the memory controller can cooperatively map the data blocks in an appropriate manner that is amenable to bulk bitwise computation via PUM.
Another key issue is how to move partial results generated in one DRAM subarray to other DRAM subarrays to continue the execution with other input operands residing in those subarrays. Several of our recent works~\cite{seshadri2013rowclone,chang.hpca14,rezaei2020nom,wang2020figaro} %\om{JUAN:ALso cite figaro} 
propose mechanisms for in-DRAM internal data movement that can facilitate gathering of data in appropriate rows/subarrays/banks in a DRAM chip.
%For instance, 

Programmer-transparent data and code mapping mechanisms are especially desirable for PIM adoption. {In~\cite{hsieh.isca16}, we present}
a software/hardware cooperative mechanism to map data and code to several
3D-stacked memory chips in regular GPU applications with relatively
regular memory access patterns. This work also deals with effectively
\emph{sharing PIM {engines} across multiple threads}, as GPU
code sections can be offloaded from different GPU cores to the PNM GPU cores in 3D-stacked memory chips.  Developing
{new approaches} to data/code mapping and scheduling for a wide
variety of applications and possible core and memory configurations is
still necessary.

In summary, there are still several key research questions that should
be investigated {in runtime systems for PIM, which perform
  scheduling and data/code mapping}:
\begin{itemize}
\item What are simple mechanisms to enable and disable PIM execution? How can PIM execution be throttled for highest performance gains? How should data locations and access patterns affect where/whether PIM execution should occur?
\item Which parts of {a given application's} code should be executed on PIM? What are simple mechanisms to identify when those parts of the application code can benefit from PIM?
\item What are scheduling mechanisms to share PIM {engines} between multiple requesting cores to maximize \chvii{benefits obtained from PIM}? 
\item What are simple mechanisms to {manage access to a memory that serves both CPU requests and PIM requests?}
%ensure Quality of Service (QoS) for memory accesses from cores and from PIM?}
\end{itemize}



\subsection{Memory Coherence}
\label{sec:coherence}
%\addcontentsline{toc}{part}{Memory Coherence}

%\jgl{Update with CoNDA.}\om{JUAN: can you revise to replace LazyPIM with CoNDA? Try to keep the changes minimal.}\om{JUAN: Also, please see what we can pull in from the IBM JRD paper. I do not want to make the CoNDA section as long as in that paper, though.}

In a traditional multithreaded execution model that makes use of
shared memory, writes to memory must be coordinated between multiple
CPU cores, to ensure that threads do not operate on stale data values.
Since CPUs include per-core private caches, when one core writes data
to a memory address, cached copies of the data held within the caches
of other cores must be updated or invalidated, using a
{mechanism} known as \emph{cache coherence}.  Within a modern
chip multiprocessor, the per-core caches perform coherence actions
over a shared interconnect, with hardware coherence protocols.

Cache coherence is a major system challenge for enabling PIM
architectures as general-purpose execution engines, as \chiii{PIM
  processing logic} can modify the data \chiii{it processes}, and this
data may also be needed by CPU cores.  If \chiii{PIM processing logic
  is} coherent with the processor, the PIM programming model is
relatively simple, as it remains similar to conventional \ch{shared
  memory} multithreaded programming\ch{, which makes PIM architectures
  easier to adopt in general-purpose systems}.  Thus, allowing
\chiii{PIM processing logic} to maintain such a simple and traditional
shared memory programming model can facilitate the \ch{widespread}
adoption of PIM.  However, employing traditional fine-grained cache
coherence {(e.g., a cache-block based MESI
  protocol~\cite{mesi1984})} for PIM forces a large number of
coherence messages to traverse {the narrow processor-memory
  bus}, potentially undoing the benefits of high-bandwidth \chvi{and
  low-latency} PIM \chv{execution}.  \chv{Unfortunately,} solutions
for coherence proposed by prior PIM
works~\cite{ahn.pei.isca15,hsieh.isca16,ahn.tesseract.isca15} either place some
restrictions on the programming model (by eliminating coherence and
requiring message passing based programming) or limit the performance
\ch{and energy} gains achievable by a PIM architecture.

We have developed a new coherence protocol,
%LazyPIM
\emph{CoNDA}~\cite{boroumand2019conda,boroumand2016pim,boroumand.arxiv17}, that maintains
cache coherence between PIM processing logic and CPU cores
\emph{without} sending coherence requests for every memory access.
%Instead, %LazyPIM 
%CoNDA efficiently provides coherence by having PIM processing logic \emph{speculatively} acquire coherence permissions, and then later sends compressed \emph{batched} coherence lookups to the CPU to determine whether or not its speculative permission acquisition violated the {coherence semantics.}  
Instead, as shown in Figure~\ref{fig:conda}, CoNDA enables efficient coherence by having the
PIM logic:
\begin{enumerate}
\item \emph{speculatively} acquire coherence permissions for multiple memory operations over a given period of time (which we call \emph{optimistic execution}; \circled{1} in the figure);
\item \emph{batch} the coherence requests from the multiple memory operations into a set of compressed coherence \emph{signatures} (\circled{2} and 
\circled{3});
\item send the signatures to the CPU to determine whether the speculation violated any coherence semantics.
\end{enumerate}
Whenever the CPU receives compressed signatures from the PIM core (e.g., when the PIM kernel finishes), the CPU performs \emph{coherence resolution} (\circled{4}), where it checks if any coherence conflicts occurred. If a conflict exists, any dirty cache line in the CPU that caused the conflict is flushed, and the PIM core rolls back and re-executes the code that was optimistically executed.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/conda-operation.pdf}
\vspace{-5mm}
\caption{High-level operation of CoNDA, a new coherence mechanism for near-data accelerators, including PNM and PUM. Reproduced from~\cite{ghose2019arxiv}. Originally presented in~\cite{boroumand2019conda}.}
\label{fig:conda}
\end{figure}


As a result {of this "lazy" checking of coherence violations}, CoNDA approaches near-ideal coherence behavior: {the performance and energy consumption of a PIM architecture with CoNDA are, respectively, within 10.4\% and 4.4\% the performance and energy consumption of} a system where coherence is performed at zero latency and energy cost.
%\jgl{We can use Figure 7 of the JRD paper and extend the explanation about the protocol.}
%\om{JUAN: Yes, can you do that? Also, please check the 5.5 and 4.4 percent numbers.}

{Despite the leap that
  CoNDA~\cite{boroumand2019conda,boroumand2016pim,boroumand.arxiv17} represents for
  memory coherence in computing systems with PIM support, we believe
  that it is still necessary to explore other solutions for memory
  coherence that can efficiently deal with all types of workloads and
  PIM offloading granularities as well as different approaches to PIM.}


\subsection{Virtual Memory Support}
\label{sec:virtualmemory}
%\addcontentsline{toc}{part}{Virtual Memory Support}

%\jgl{We can incorporate reference to VBI.}\om{JUAN: Agreed. Please do. Please also see if we can incorporate good stuff from the JRD paper.}

When an application needs to access its data inside the main memory,
the CPU core must first perform an \emph{address translation}, which
converts the data's virtual address into a \emph{physical} address
within main memory.  If the translation {metadata} is not
available in the CPU's translation lookaside buffer (TLB), the CPU
must invoke the page table walker in order to perform a long-latency
page table walk that involves multiple \emph{sequential} reads to the
main memory and lowers the application's performance. In modern
systems, the virtual memory system also provides access protection
mechanisms.

%\todo 
%A large amount of code relies on pointers, which are stored as
%\emph{virtual} memory addresses.  
%\ch{When the application follows a pointer, a core must perform \emph{address translation},
%which converts the pointer's stored virtual address into a \emph{physical} address within main memory.}
%% In order to access the data that is being
%% pointed to by these virtual addresses, a core needs to perform \emph{address
%% translation} in order to find the \emph{physical} address, as main memory \rachata{itself} is
%% physically addressed.
%If \chiii{PIM processing logic} relies on
%  existing CPU-side address translation mechanisms, any performance
%  gains from performing pointer chasing in memory could easily be
%  nullified, as the \chiii{processing logic} needs to send a
%    long-latency translation request to the CPU via the off-chip channel for each memory access.  
%    The translation can sometimes require a page table walk, where
%    the CPU must issue \ch{\emph{multiple}} memory requests to read the page table, which
%    further increases traffic on the memory channel.
  %   This
  % request can result in a page table walk that issues multiple memory
  % requests back to the memory, thereby leading to increased memory
  % traffic on the main memory channels. 


A naive solution to reducing the overhead of page walks is to utilize
PIM engines to perform page table walks. This can be done by
duplicating the content of the TLB and {moving} the page walker
{to} the PIM processing logic in main memory.  Unfortunately,
this is either difficult or expensive for three reasons. First,
coherence {has} to be maintained between the CPU's TLBs and the
memory-side TLBs. This introduces extra complexity and off-chip
requests.  Second, duplicating the TLBs increases the storage and
complexity overheads {on the memory side, which should be
  carefully contained}.  Third, if main memory is shared across
{CPUs with} different types of architectures, page table
structures and the implementation of address translations can be
different across {the different} architectures. Ensuring
compatibility between the in-memory TLB/page walker and all possible
types of {virtual memory} architecture designs can be
complicated and often not even practically feasible.

To address these concerns and reduce the overhead of virtual memory,
we explore a tractable solution for PIM address translation as part of
our in-memory pointer chasing accelerator, IMPICA~\cite{impica}.
IMPICA exploits the high bandwidth available within 3D-stacked memory
to traverse a chain of virtual memory pointers within DRAM,
\emph{without} having to look up virtual-to-physical address
translations in the CPU translation lookaside buffer (TLB) and without
using the page walkers within the CPU.  {IMPICA's key ideas are
  1) to use a region-based page table, which is optimized for PIM
  acceleration, and 2) to decouple address calculation and memory
  access with two specialized engines.  IMPICA improves the
  performance of pointer chasing operations in three commonly-used
  linked data structures (linked lists, hash tables, and B-trees) by
  92\%, 29\%, and 18\%, respectively. On a real database application,
  DBx1000, IMPICA improves transaction throughput and response time by
  16\% and 13\%, respectively. IMPICA also reduces overall system
  energy consumption (by 41\%, 23\%, and 10\% for the three
  commonly-used data structures, and by 6\% for DBx1000).}

Beyond pointer chasing operations that are tackled by
IMPICA~\cite{impica}, providing efficient mechanisms for PIM-based
virtual-to-physical address translation (as well as access protection)
remains a challenge for the generality of applications,
especially those that access large amounts of virtual
memory~\cite{mask,mosaic,mosaic-osr}.  %We believe it is important to
%explore new ideas to address this PIM challenge in a \sg{scalable and}
%efficient manner.

Looking forward, we recently introduced a fundamentally-new virtual memory framework, the Virtual Block Interface (VBI)~\cite{hajinazar2020virtual}, which proposes to delegate physical memory management duties completely to the memory controller hardware as well as other specialized hardware. 
Figure~\ref{fig:vbi} compares VBI to conventional virtual memory at a very high level.
Designing VBI-based PIM units that manage memory allocation and address translation can help fundamentally overcome this important virtual memory challenge of PIM systems. We refer the reader to our VBI work~\cite{hajinazar2020virtual} for details.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/vbi.pdf}
\vspace{-5mm}
\caption{The Virtual Block Interface versus conventional virtual memory. Reproduced from~\cite{hajinazar2020virtual}.}
\label{fig:vbi}
\end{figure}


\subsection{Data Structures for PIM}
\label{sec:datastructures}
%\addcontentsline{toc}{part}{Data Structures for PIM}

Current systems with many cores run applications with concurrent data
structures to achieve high performance and scalability, with
significant benefits over sequential data structures. Such concurrent
data structures \sg{are often used in} % which are especially in
heavily-optimized server systems today, where high performance is
critical. To enable the adoption of PIM in such many-core systems, it
is necessary to develop concurrent data structures that are
specifically tailored to take advantage of PIM.

\emph{Pointer chasing data structures} and \emph{contended data
  structures} require careful analysis and design to leverage the high
bandwidth and low latency of 3D-stacked memories~\cite{liu-spaa17}.
First, pointer chasing data structures, such as linked-lists and
skip-lists, have a high degree of inherent parallelism and low
contention, but a naive implementation in PIM cores is burdened by
hard-to-predict memory access patterns. By combining and partitioning
the data across 3D-stacked memory vaults, it is possible to fully
exploit the inherent parallelism of these data structures.  Second,
contended data structures, such as FIFO queues, are a good fit for CPU
caches because they expose high locality. However, they suffer from
high contention when many threads access them concurrently.
{Their performance on traditional CPU systems can be improved
  using a new PIM-based FIFO queue~\cite{liu-spaa17}.  The proposed
  PIM-based FIFO queue uses a PIM core to perform enqueue and dequeue
  operations requested by CPU cores. The PIM core can pipeline
  requests from different CPU cores for improved performance.}

{As \sg{recent work~\cite{liu-spaa17}} shows, PIM-managed concurrent data
  structures can outperform state-of-the-art concurrent data
  structures that \sg{are designed} for and executed on multiple cores. We
  believe and hope that future work will enable other types of data
  structures (e.g., hash tables, search trees, priority queues) to
  benefit from PIM-managed designs.}


\subsection{Benchmarks and Simulation Infrastructures}
\label{sec:simulation}
%\addcontentsline{toc}{part}{Benchmarks and Simulation Infrastructures}

%\jgl{We can extend this section with Ramulator-PIM and NAPEL.}\om{JUAN: Agreed. Please do. Can you go over the entore section and update it with the above two works + PIM-WL paper description and citations. I started a bit but prefer that you take a cut first here and then I will look over, hopefully tomorrow (Thursday oct 29)}

%\todo
%\chii{To ease adoption, it is critical that \chiii{we accurately} assess the benefits
%of PIM.  Accurate assessment for PIM requires
%(1)~a set of real-world memory-intensive applications that have the potential to benefit significantly when executed near memory, and
%(2)~a \chiii{simulation/evaluation} infrastructure that allows architects and system designers to
%precisely analyze the benefits and overhead of adding \chiii{PIM processing logic} to memory and
%executing code on \chiii{this processing logic}}.

To ease the adoption of PIM, it is critical that we {accurately}
assess the benefits and shortcomings of PIM. Accurate assessment of
PIM requires (1)~a {preferably large} set of real-world
memory-intensive applications that have the potential to benefit
significantly when executed near memory, (2)~a rigorous methodology to
(automatically) identify PIM offloading candidates, and
(3)~simulation/evaluation infrastructures that allow architects and
system designers to {accurately} analyze the benefits and
overheads of adding PIM processing logic to memory and executing code
on this processing logic.

%\todo
%\ch{\chii{In order to identify what \chiii{processing logic} should be introduced near memory, and 
%to know what properties are ideal for PIM kernels, we must begin by developing a
%real-world benchmark suite of applications that can potentially benefit from PIM.
% An upcoming challenges to PIM is the lack of a real-world benchmark suite that takes advantage of PIM. 
%\chvii{While many data-intensive applications, such as pointer chasing and bulk memory copy,
%can potentially benefit from PIM,} it is crucial to examine important candidate applications for PIM
%execution, and for researchers to agree on a common set of these candidate applications
%to focus the efforts of the community.  
%We believe that these applications should come from a number of popular and emerging
%domains.  Examples of potential domains include} data-parallel applications, neural networks, 
%\chiii{machine} learning, graph processing, \chiii{data analytics,} search/filtering, mobile workloads, bioinformatics, Hadoop/Spark programs, and in-memory data stores.  
%\chiii{Many of these} applications have large data sets and can
%benefit from high memory bandwidth and low memory latency benefits provided by
%PIM mechanisms.}
% It is important to analyze these diverse programs to identify the kernels
% suitable for PIM.  These kernels and applications can also be used as a
% benchmark suite for evaluating PIM performance/efficiency. 
%\chii{As an example, in
%our prior work, we have started analyzing mechanisms for accelerating graph
%processing~\cite{ahn.pei.isca15,ahn.tesseract.isca15};
%pointer chasing~\cite{cont-runahead,impica};
%\chiii{databases~\cite{boroumand2016pim, boroumand.arxiv17, impica, GS-DRAM};} 
%consumer workloads~\cite{boroumand.asplos18}, including web browsing,
%video encoding/decoding, and machine learning;
%and GPGPU workloads~\cite{hsieh.isca16,pattnaik.pact16}.}

In order to explore what processing logic should be introduced near
memory, and to know what properties are ideal for PIM kernels, we
believe it is important to begin by developing a \emph{real-world
  benchmark suite} of a wide variety of applications that can
potentially benefit from PIM. While many data-intensive applications,
such as pointer chasing and bulk memory copy, can potentially benefit
from PIM, it is crucial to examine important candidate applications
for PIM execution, and for researchers to agree on a common set of
these candidate applications to focus the efforts of the community
{as well as to enable reproducibility of results, which is
  important to assess the relative benefits of different ideas
  developed by different researchers}. We believe that these
applications should come from a number of popular and emerging
domains. Examples of potential domains include data-parallel
applications, neural networks, machine learning, graph processing,
data analytics, search/filtering, mobile workloads, bioinformatics,
Hadoop/Spark programs, security/cryptography, and in-memory data
stores. Many of these applications have large data sets and can
benefit from high memory bandwidth and low memory latency benefits
provided by computation near memory. In our prior work, we have
started identifying several applications that can benefit from PIM in
graph processing
frameworks~\cite{ahn.pei.isca15,ahn.tesseract.isca15}, pointer
chasing~\cite{cont-runahead,impica}, databases~\cite{boroumand2016pim,boroumand2019conda,boroumand.arxiv17, impica, GS-DRAM}, consumer workloads~\cite{boroumand.asplos18}, 
time series analysis~\cite{fernandez2020natsa}, genome analysis~\cite{kim.bmc18,cali2020genasm}, 
machine learning~\cite{boroumand.asplos18}, and GPGPU
workloads~\cite{hsieh.isca16,pattnaik.pact16}.  {However, there
  is significant room for methodical development of a large-scale PIM
  benchmark suite, which our very recent work~\cite{oliveira2021pimbench}
  %\om{JUAN: cite PIM WL} 
  takes the first steps for.}

%\todo
%\chii{Once we have established a set of applications to explore,
%it is essential for researchers to develop an extensive and flexible application profiling and simulation
%infrastructure and mechanisms that can (1)~identify parts of these applications
%for which PIM execution can be beneficial; and
%(2)~simulate in-memory acceleration.
%A systematic process for identifying potential PIM kernels within an application can not only ease
%the burden for performing PIM research, but could also inspire tools that 
%programmers and compilers can use to automate the process of offloading portions
%of existing applications to \chiii{PIM processing logic}.
%Once we have identified potential PIM kernels, we need a simulator to accurately model 
%the energy and performance consumed by PIM hardware structures, 
%available memory bandwidth, and communication overhead when
%we execute the kernels near memory.}
% of such
% application portions is also an important research topic for PIM. 
%\chii{Highly-flexible memory} simulators (e.g., Ramulator\chiii{~\cite{ramulator, ramulator.github}}, SoftMC\chiii{~\cite{hassan2017softmc, softmc.github}})
%\chii{can be combined} with full-system simulation infrastructures (e.g., gem5~\cite{GEM5})
%\chii{to} provide a robust environment \chii{that can} evaluate how various PIM architectures
%affect the \chii{\emph{entire compute stack}, and can allow designers to
%identify memory characteristics (e.g., internal bandwidth, trade-off between number
%of PIM engines and memory capacity) that affect the efficiency of PIM execution}.
% There is a need to develop profiling and simulation tools at
% multiple abstraction layers which can evaluate both modern
% data-intensive workloads as well as emerging workloads.


A systematic \emph{methodology} for (automatically) identifying
potential PIM kernels (i.e., code portions that can benefit from PIM)
within an application can, {among many other benefits, 1) ease
  the burden of programming PIM architectures by aiding the programmer
  to identify what should be offloaded, 2) ease the burden of and
  improve the reproducibility of PIM research, 3) drive the design and
  implementation of PIM functional units that many types of
  applications can leverage, 4) inspire the development of tools that
  programmers and compilers can use to automate the process of
  offloading portions of existing applications to PIM processing
  logic, and 5) lead the community towards convergence on PIM designs
  and offloading candidates.} In a very recent work that is to appear in 2021~\cite{oliveira2021pimbench},
  %\om{JUAN: cite PIM WL}, 
  we take the first steps in developing such a methodology and the first benchmark suite for PIM. We refer the reader to that work~\cite{oliveira2021pimbench}
  %\om{JUAN: cite PIM WL}
  for detailed description and analyses of the methodology and the new PIM benchmark suite. We believe this work opens up many more steps to extend the methodology and develop other new methodologies for identifying PIM kernels as well as automatic tools (e.g., profilers, compilers, runtime systems) that implement these methodologies, generate optimized code for PIM (potentially with help from programmer annotations), coordinate offloading to PIM cores, etc.

Along these lines, our NAPEL~\cite{singh2019napel} work is an early example of an ML-based performance and energy estimation framework for PNM. NAPEL leverages ensemble learning techniques to generate PNM performance and energy prediction models that are based on microarchitecture parameters and application characteristics. Figure~\ref{fig:napel} shows the high-level overview of NAPEL training and prediction, the components of which are explained in detail in~\cite{singh2019napel}. 
Our evaluations show that NAPEL can make fast yet accurate predictions of PIM offloading suitability for previously-unseen applications on general-purpose PNM architectures.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/ModelEmbed.pdf}
\vspace{-5mm}
\caption{Overview of NAPEL training and prediction. Components are explained in detail in~\cite{singh2019napel}. Figure reproduced from~\cite{singh2019napel}.}
\label{fig:napel}
\end{figure}


%\om{JUAN: Update with NAPEL and Ramulator-PIM} %JGL-2020-1029
{We also} need \emph{simulation infrastructures} to accurately
model the performance and energy of PIM hardware structures, available
memory bandwidth, and communication overheads when we execute code
near or inside memory. Highly-flexible and commonly-used memory
simulators (e.g., Ramulator~\cite{ramulator, ramulator.github},
SoftMC~\cite{hassan2017softmc, softmc.github}) can be combined with
full-system simulators (e.g., gem5~\cite{GEM5}, zsim~\cite{zsim},
gem5-gpu~\cite{gem5-gpu}, GPGPUSim~\cite{gpgpusim}) to provide a
robust environment that can evaluate how various PIM architectures
affect the \emph{entire compute stack}, and can allow designers to
identify memory, workload, and system characteristics that affect the
efficiency of PIM execution. %We believe it is critical to support the
%open source development such \sg{simulation and} emulation infrastructures
%for assessing the benefits of a wide variety of PIM designs.
A powerful open-source simulation infrastructure that provides such environment is Ramulator-PIM~\cite{ramulator-pim}, first introduced by our NAPEL framework~\cite{singh2019napel}, which combines Ramulator~\cite{ramulator, ramulator.github} and zsim~\cite{zsim}. %\om{JUAN: Please cite zsim paper}. 
Ramulator-PIM can simulate a wide range of configurations of PIM in-order and out-of-order cores and accelerators with different memory technologies.


\subsection{Real PIM Hardware Systems and Prototypes}
\label{sec:realpim}
%\addcontentsline{toc}{part}{Real PIM Hardware Systems and Prototypes}

As industry and academia push toward enabling the PIM paradigm, it will be important to also provide real PIM hardware or prototypes. Such hardware can greatly enable and accelerate evaluations of both adoption and research issues in PIM, leading to learnings from real workloads executed on real systems and thus better PIM systems over time. Such real hardware for PIM is very much useful for both PUM and PNM approaches. 

We are aware of at least two such real hardware systems. First, ComputeDRAM~\cite{gao2020computedram},
%\om{JUAN: Please cite}, 
which is based on the SoftMC memory controller infrastructure~\cite{hassan2017softmc}  %\om{JUAN: Please cite} 
can potentially provide the opportunity to test Rowclone (Section~\ref{sec:rowclone})  %\om{JUAN: ref}) 
and Ambit (Section~\ref{sec:ambit}) 
%\om{JUAN: ref}) 
PUM approaches on real workloads, albeit likely at reduced reliability since it exploits off-the-shelf DRAM chips, as we discussed in Section~\ref{sec:ambit}.
%\om{JUAN: ref}. 

Second, the recent UPMEM PIM architecture~\cite{upmem2018, devaux2019}, shown in Figure~\ref{fig:upmem} is the first real-world publicly-available PIM architecture. This PNM system consists of one simple processors (called DRAM Processing Unit, DPU) implemented next to each bank in a DRAM chip. A DPU has high-bandwidth, low-latency, low-energy access to all the data in its corresponding bank. UPMEM has produced real DRAM modules that contain 
16 PNM-capable DRAM chips each. Each DRAM chip includes eight 64-MB DRAM banks, each of which has a DPU attached running at a few hundred MHz. A full-blown UPMEM system configuration is expected to soon have 2560 DPUs capable of operating on 160 GB of DRAM memory.  We believe the existence of such real PIM hardware can greatly enable and accelerate software and adoption-related research for PIM, specifically PNM architectures, and can set a promising and useful baseline for future research in PNM systems.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{PIM_MST_MicPro2018/figures/upmem.pdf}
\vspace{-5mm}
\caption{UPMEM PIM architecture and hardware. Reproduced from~\cite{mutlu.nsfpim20}.}
\label{fig:upmem}
\end{figure}


\subsection{Security Considerations}
\label{sec:security}
%\addcontentsline{toc}{part}{Security Considerations}

As a new processing paradigm, PIM introduces new security considerations related to its integration in real-world computing systems. 
First, there is a need to provide security guarantees in systems with PIM capabilities so that applications that offload code can execute securely in PIM computation units. Naively providing access to PIM computation units for all concurrently-executing applications may lead to potentially unforeseen data leakage and other issues. Second, the ability to perform computation inside or near memory using PIM can enable the opportunity to specialize such computation mechanisms to enhance system security (as briefly discussed in Section~\ref{sec:puf-trng}). 
%\om{JUAN:Please Ref to the in-dram sec primitives section.}) 
We cover each of these topics briefly but envision many future ideas related to them in future PIM research and designs. 

First, PIM computation units should provide at least as good security primitives as processor-centric computation units of today. This means that there should at least be isolation between concurrently-executing processes on PIM computation units and access control to PIM resources (both data storage and computation units) should be securely managed. Partitioning of computation units, as done in ~\cite{hajinazar2020virtual}, can enable isolation. We believe new approaches to virtualization and cross-layer design that provide extensive hardware management capabilities in the memory controllers, such as the Virtual Block Interface (VBI)~\cite{hajinazar2020virtual} or Expressive Memory~\cite{vijaykumar2018xmem,vijaykumar2018locality} 
%\om{JUAN: Please cite Xmem and Locality descriptor papers} 
can not only make PIM security mechanisms easier and more effective to implement but can provide much more enhanced PIM security mechanisms than existing systems. 

As in existing systems, \emph{reliability} and \emph{data integrity} are important in PIM systems, especially in PUM approaches, where memory rows can be frequently activated and deactivated. The RowHammer vulnerability~\cite{kim-isca2014,mutlu2017rowhammer,mutlu2020retrospective,kim2020revisiting,cojocar2020susceptible,frigo2020trr} 
%\om{JUAN: Also cite our DATE 2017, TCAD 2019, ISCA 2020, S\&P 2020 papers}
(Section~\ref{sec:majortrends}) 
%\om{JUAN: please ref}) 
can potentially become exacerbated in PIM systems but it can also be more easily preventable using an intelligent memory controller as in PIM. The cell wearout problem due to endurance limitations in some modern NVM technologies can limit the reliability and thus effectiveness of NVM-based PUM approaches~\cite{kvatinsky.iccd11,kvatinsky.tcasii14,kvatinsky.tvlsi14,li.dac16,bhattacharjee2017revamp} and thus needs to be addressed. Employing in-memory error correcting code (ECC) \rachata{techniques~\cite{binarystar,patel2019understanding,patel2020bit}} %RA: added binarystar
is likely necessary in future PIM approaches and PIM systems should likely be designed to support ECC techniques to maintain data reliability in the presence of computation mechanisms using/near memory and increasing noise and reliability problems due to technology scaling.

Second, the PIM paradigm enables new opportunities to increase the security and privacy of computations and data, and thus entire computing systems. If data and computation stay within one chip, then the exposure of such data and computation to many attacks will likely be minimized. By eliminating data movement between memory and processor, the PIM paradigm takes a large step towards getting rid of one of the most attacker-exposed type of  data movement, i.e., data movement over the main memory bus. Enabling the secure and private execution of computations in PIM systems can therefore potentially enable fundamentally more secure computing systems. This requires providing support for such secure computation, as we discussed earlier in Section~\ref{sec:puf-trng}. 
%\om{JUAN: please cite the in-DRAM security primitives section}. 
For example, our afore-described DRAM latency PUF~\cite{kim.hpca18} and DRAM latency True Random Number Generator~\cite{kim.hpca19} are notable examples of novel in-DRAM security primitives that take advantage of Processing Using Memory that were  briefly discussed in Section~\ref{sec:puf-trng}. 
%\om{JUAN:Please Ref to the in-dram sec primitives section.}. 
We envision future works on PIM will provide many other security primitives, applications, and use cases.



%\addcontentsline{toc}{part}{Conclusion and Future Outlook}

Data movement is a major performance and energy bottleneck plaguing
modern computing systems. A large fraction of system energy is spent
on moving data across the memory hierarchy into the processors (and
accelerators), the only place where computation is performed in a
modern system. Fundamentally, the large amounts of data movement \sgii{are}
caused by the processor-centric design paradigm of modern computing systems:
processing of data is performed only in the processors (and
accelerators), which are far away from the data, and as a result, data
moves a lot in the system, to facilitate computation on it.

In this work, we argue for a paradigm shift in the design of computing
systems toward a data-centric design paradigm that enables computation
capability in places where data resides and thus performs computation
with minimal data movement.  \sg{\emph{Processing-in-memory} (PIM) is
  a fundamentally data-centric design approach for computing systems
  that enables the ability to perform operations in or near memory.
  Recent advances in modern memory architectures have enabled us to
  extensively explore two novel approaches to designing PIM
  architectures: PUM (Processing Using Memory) and PNM (Processing Near Memory).  First, we show that PUM exploits the existing DRAM architecture and the operational principles of the DRAM circuitry, enabling a number of important and widely-used operations
  (e.g., memory copy, data initialization, bulk bitwise operations,
  data reorganization) within DRAM, with minimal changes to DRAM chips. Similar PUM approaches are also applicable to other types of memory chips, and all yield large performance and energy benefits.  Second, we demonstrate that PNM can exploit the
  embedded computation capability in the logic layer of 3D-stacked
  memory in a variety of ways to provide significant
  performance improvements and energy savings, across a large range of
  application domains and computing platforms. Similar PNM approaches are applicable to different types of memories and also to memory controllers.}


%%% ONUR: I wrote the above paragraphs, but did not get a chance to continue. @SAUGATA: Can you continue from what I started?
%%% ONUR: I would like to reiterate the points I made in my conclusion slide of my recent GWU distinguished lecture. The conclusion does not need to be long. It needs to be powerful. 

%%%ONUR: The below paragraphs are a different style. Thye can be
%%%useful, but I would like to make the conclusion much stronger...



%{We presented recent efforts to enable Processing-in-Memory for
%  a wide variety of computing systems}.  We have identified data
%movement as the major {performance and energy} bottleneck in
%current computing systems.  {Data movement is greatly
  %exacerbated in current systems due to the processor-centric design
%  paradigm, where all data needs to be brought to the processor before
%  it can be operated on.}  Processing-in-Memory avoids the pitfalls of
%processor-centric architectures by {enabling computation
%  capability inside or near main memory}, which is a paradigm shift
%from the processor-centric nature of modern computing systems.

%%% ONUR: This needs a lot more work to be crisp. Key conclusions are not coming out. @Saugata: Can you handle this?
% We have presented two {new approaches to designing PIM
%   architectures}.  First, we have shown that, {with minimal
%   changes to memory chips, it is possible to execute important
%   memory-intensive operations (e.g., memory copy, initialization, bulk
%   bitwise operations, and data reorganization) within DRAM at low cost
%   and at very high performance and efficiency.}  {Second, we
%   have shown the extensive design space exploration that we carry out
%   for embedding compute capability in the logic layer of 3D-stacked
%   memory. Our works span from coarse-grained accelerators for graph
%   processing (i.e., Tesseract) to fine-grained instruction offloading
%   (i.e., PEI). We also propose efficient designs for functions that
%   suffer from the data movement bottleneck in consumer workloads and
%   in GPU applications.}

%%% ONUR: This needs a lot more work to be crisp. It isnot comprehensive and it sounds naive. @Saugata: Can you handle this?
\sg{Despite the extensive design space that we have studied so far, a
  number of key challenges remain to enable the widespread adoption of
  PIM in future computing systems~\cite{ghose.bookchapter19,
    ghose.bookchapter19.arxiv}.}  \sg{Important challenges include
  developing easy-to-use programming models for PIM (e.g., PIM
  application interfaces, compilers and libraries designed to abstract
  away PIM architecture details from programmers), and extensive
  runtime support for PIM (e.g., scheduling PIM operations, sharing
  PIM logic among CPU threads, cache coherence, virtual memory
  support).}  We \sg{hope} that providing the community with (1)~a
large set of memory-intensive benchmarks that can potentially benefit
from PIM, (2)~a rigorous methodology to identify PIM-suitable parts
within an application, and (3)~accurate simulation infrastructures for
estimating the benefits and overheads of PIM will empower researchers
to address \sg{remaining} challenges for the adoption of PIM.
  
\juan{We firmly believe that it is time to design principled system
  architectures to solve the data movement problem of modern computing
  systems, which is caused by the rigid dichotomy and imbalance
  between the computing unit (CPUs and accelerators) and the
  memory/storage unit. Fundamentally solving the data movement problem
  requires a paradigm shift to a more data-centric computing system
  design, where computation happens where data resides (i.e., in or near memory/storage), with
  minimal movement of data.  Such a paradigm shift can greatly push
  the boundaries of future computing systems, leading to orders of
  magnitude improvements in energy and performance (as we demonstrated
  with some examples in this work), potentially enabling new
  applications and computing \sgii{platforms.}}
  % , and likely helping to solve
  % many challenges to better understand nature.}

%\om{JUAN: please cite our DAC 2019 short paper + My vLSI DAT/TSA 2020 keynote paper at appropriate places in the document.} \jgl{Both cited in intro, with the MicPro paper.}
